SIFU: Sequential Informed Federated Unlearning for Efficient and Provable Client Unlearning in Federated Optimization

Machine Unlearning (MU) is an increasingly important topic in machine learning safety, aiming at removing the contribution of a given data point from a training procedure. Federated Unlearning (FU) consists in extending MU to unlearn a given client's contribution from a federated training routine. While several FU methods have been proposed, we currently lack a general approach providing formal unlearning guarantees to the FedAvg routine, while ensuring scalability and generalization beyond the convex assumption on the clients' loss functions. We aim at filling this gap by proposing SIFU (Sequential Informed Federated Unlearning), a new FU method applying to both convex and non-convex optimization regimes. SIFU naturally applies to FedAvg without additional computational cost for the clients and provides formal guarantees on the quality of the unlearning task. We provide a theoretical analysis of the unlearning properties of SIFU, and practically demonstrate its effectiveness as compared to a panel of unlearning methods from the state-of-the-art.

==> tex/DP.tex <==
Differential privacy (DP) is commonly used in FL to guarantee a level of anonymity to every client data in the learnt model. With a DP algorithm, obtaining a model with every client has a similar probability to obtaining it with every client but one. The output of a DP algorithm must satisfy Definition \ref{def:DP_forget} for any output trained with $\Dcal$ and $\Dcal_{-m}$.
\begin{definition}[$(\epsilon, \delta)$-indistinguishable] 
	For $\epsilon \ge 0$ and $\delta \ge 0$, two distributions $X$ and $Y$ are $(\epsilon, \delta)$-indistinguishable if for all subset $A \subseteq Range(X)\cup Range(Y)$, we have
	\label{def:DP_forget}
	\begin{equation}
	\mathbb{P}(X \in A) 
	\le e^\epsilon \mathbb{P}(Y \in A)  + \delta
	\end{equation}
	\begin{equation}
	\text{and }
	\mathbb{P}(Y \in A) 
	\le e^\epsilon \mathbb{P}(X \in A)  + \delta
	.
	\end{equation}
\end{definition}
A model satisfying DP has degraded performance to satisfy the data privacy level monitored through the privacy parameters $\epsilon$ and $\delta$. To satisfy $(\epsilon, \delta)$-DP, the learning procedure must be designed for the client dataset with the most data specificity. With Definition \ref{def:DP_adpated}, we propose instead the following criterion ensuring that the learning procedure is modified solely to accommodate the clients to forget.
\begin{definition}[$(\epsilon, \delta)$-forgetting of client $m$]\label{def:DP_adpated}
	Let us consider a randomized algorithm $\Mcal$. If $\Mcal(\Dcal)$ and $\Mcal(\Dcal_{-m})$ are $(\epsilon, \delta)$-indistinguishable, client $m$ has been forgotten from $\Mcal(\Dcal)$. 
\end{definition}
If a learning procedure satisfies Definition \ref{def:DP_adpated} for every client, then the returned model is also $(\epsilon, \delta)$-DP. Satisfying Definition \ref{def:DP_adpated} is weaker than satisfying DP privacy.

%\begin{definition}[Forgetting client $k$]\label{def:DP_adpated}
%	A randomized algorithm $\Mcal$ is $(\epsilon, \delta)$-differentially private if for all $\Scal \subseteq \text{Range}(\Mcal)$ and for $\vx, \vy \in \{\Dcal, \Dcal_{-k}\}$, we have
%	\begin{equation}
%		\mathbb{P}\left[\Mcal(\vx) \in \Scal\right]
%		\le e^{\epsilon} \mathbb{P}\left[\Mcal(\vy) \in \Scal\right]
%		+ \delta
%		.
%	\end{equation} 
%	
%\end{definition}

%Definition \ref{def:DP_adpated} is adapted to the unlearning setting. The dataset difference is only the one of the client we want to forget, and not the one of every client.






















==> tex/SIFU_example.tex <==
\input{./tex/example_SIFU}

We consider an example of SIFU, where the server receives sequentially $R=3$ forgetting requests for one client, in Figure \ref{fig:example_with_R3}. We first describe SIFU behavior for $r=0$ and $r=1$, which is identical to IFU, Algorithm \ref{alg:unlearning_ours} in Section \ref{subsec:unlearning_ours}. Finally, we describe SIFU behavior for new forgetting requests ($r=2$ and $r=3$).  

At $r=0$, the server trains with \textsc{FedAvg} and clients in $I$ up until, after $N_0$ server aggregations, the server has the desired performances. We now consider an oracle keeping 

At $r=1$, we initialize the oracle keeping track of the noise perturbation with the initial mod

The oracle is initialized with $O(0) = \{(0,0)\}$. At $r=1$, the server forgets clients in $W_1$. The metric of clients in $W_1$ are inferior to $\Psi^*$ in $\vtheta_0^0$ (by construction). Hence, the server picks the global model with highest amount of server aggregations $n$ in the training $r=0$ such that every metric for clients in $W_1$ is inferior to $\Psi^*$, and updates the oracle as $O(1) = \{(0,0), (0, 4)\}$. The server perturbs $\vtheta_0^4$ with noise of standard deviation $\sigma$ to obtain $\vtheta_1^0$. After $N_2 = 4$ server aggregations with \textsc{FedAvg} with clients in $I_1 = I \setminus W_1$, the server obtains a global model with desired performance on clients in $I_1$, while having forgot clients in $W_1$. A similar process arrives at $r=2$ to forget clients in $W_2$. Indeed, for both $\vtheta_0^0$ and $\vtheta_0^4$, the metric of clients in $W_2$ is inferior to $\Psi^*$. Clients in $W_2$ were thus $(\epsilon,\delta)$ forgotten with the ones in $W_1$. Hence, the server picks the global model at the previous forgetting index ($r=1$) with highest amount of server aggregations such that every client metric is inferior to $\Psi^*$ ($n=3$), which gives new oracle $O(1) = \{(0,0), (0, 4), (1, 3)\}$. Again, retraining to reach is performed on $N_2=4$ server aggregations with \textsc{FedAvg} on perturbed model $\vtheta_2^0$. Forgetting clients in $W_3$ si different from $W_1$ and $W_2$. Indeed, all the global models with coordinates in $O(2)$ do not $(\epsilon,\delta)$ forgets clients in $W_3$. The metric of every client in $W_3$ is inferior to $\Psi^*$ for $(0, 0)$ and $(0, 4)$ but not for $(1, 3)$. Hence, the server selects the global model with lowest forgetting index in $O(2)$ such that clients in $W_3$ metric was above $\Psi^*$ ($r=1$), instead of the previous forgetting index ($r=2$). By considering the highest amount of server aggregations at forgetting index $r=1$ such that the metric of every client in $W_3$ is inferior to $\Psi^*$, we update the oracle as $O(3) = \{(0,0), (0, 4), (1, 2)\}$.
		

==> tex/acknowledgements.tex <==
\section*{Acknowledgements and Disclosure of Funding}
\label{sec:ack}

This work has been supported by the French government, through the 3IA Côte d’Azur Investments in the Future project managed by the National Research Agency (ANR) with the reference number ANR-19-P3IA-0002, and by the ANR JCJC project Fed-BioMed 19-CE45-0006-01. The project was also supported by Accenture.
% and the Inria Sophia Antipolis - Méditerranée, “NEF" computation cluster.
The authors are grateful to the OPAL infrastructure from Université Côte d'Azur for providing resources and support.

==> tex/alternative_SGD.tex <==
\section{Alternative SGD}

We first formalize the learning and unlearning problem. We consider $\Lcal_1$ the averaged loss over a dataset of $n$ samples. Without loss of generality we consider removing the sample with index $n$ from the dataset which gives the new loss function $\Lcal_2$. Hence, we have
\begin{equation}
\Lcal_1(\theta)
= \frac{1}{n}\sum_{i=1}^{n} l(\theta, X_i, y_i)
\text{ and }
\Lcal_2(\theta)
= \frac{1}{n-1}\sum_{i=1}^{n-1} l(\theta, X_i, y_i)
.
\end{equation}
We denote by $\theta_1^*$ and $\theta_2^*$ the respective minimum of $\Lcal_1$ and $\Lcal_2$. For simplicity, we denote $l_i(\theta) \coloneqq l(\theta, X_i, y_i)$. Retraining is done on amount $K$ of gradient descents. In practice for computation concerns, optimizations steps have to use GD instead of SGD. Let us consider $m$ to be the batch size. The variance between the gradient estimator and the true gradient is shown to slow down the learning process. We thus propose another gradient method enabling faster optimization and thus faster unlearning. 

We can express the gradient of $\Lcal_2$ in function of the one of $\Lcal_1$ as 
\begin{equation}
\nabla\Lcal_2(\theta)
= \frac{1}{n-1}\sum_{i=1}^{n-1} \nabla l_i(\theta)
= \frac{n}{n-1} \nabla\Lcal_1 (\theta) - \frac{1}{n-1}\nabla l_n(\theta)
.
\end{equation}
We note that if the training has been properly done then the learnt model is $\theta_1^*$ and therefore, the unlearning process starts with $\nabla\Lcal_2(\theta_1^*) = - \frac{1}{n-1}\nabla l_n(\theta_1^*)$ showing that the deleted data is the only sample with importance when forgetting this sample from the learnt model.



%\begin{equation}
%g_{S_1}(\theta)
%= \sum_{i=1}^{n-1} \omega_i(S_1) \nabla l_i(\theta)
%\text{ and }
%g_{S_2}(\theta)
%= \sum_{i=1}^{n-1} \omega_i(S_2) \nabla l_i(\theta)
%+ \left(\omega_n(S_2)  + \omega_{n+1}(S_2) \right) \nabla l_n(\theta)
%\end{equation}


%Let us consider two methods to create a minibatch. For the first equation, with $S_1$ $m$ samples are uniformly selected without replacement from the $n-1$ kept samples. While with $S_2$ m samples are uniformly selected without replacement from the $n+1$ samples. Therefore a sample has probability $m/(n-1)$ to be selected in $S_1$ and $m/(n+1)$ in $S_2$. We have
%\begin{equation}
%	\omega_i(S_1) 
%	= \mathbb{I}(i\in S_1)\frac{1}{m}
%	\text{ and }
%	\omega_i(S_2) 
%	= \mathbb{I}(i\in S_2)\frac{n+1}{m}\frac{1}{n-1}
%\end{equation}
%which gives $\EE{S_1}{\omega_i(S_1)} = \EE{S_2}{\omega_i(S_2)} = \frac{1}{n-1}$. and thus prove that 
%
%$S_1$ and $S_2$. With $S_1$, $m$ samples are sampled uniformly without replacement.
%
%
%We consider the SGD variance for the two methods.
%\begin{align}
%	\norm{g_{S_2}(\theta)  - \nabla \Lcal_2(\theta)}^2
%	&= \norm{g_{S_2}(\theta)  - g_{S_1}(\theta)}^2
%	+ \norm{g_{S_1}(\theta)  - \nabla \Lcal_2(\theta)}^2
%	\nonumber\\
%	& + 2 \inner{g_{S_2}(\theta)  - g_{S_1}(\theta)}{g_{S_1}(\theta)  - \nabla \Lcal_2(\theta)}
%	\label{eq:decomposition}
%\end{align}
%$S_1$ and $S_2$ are independent and our gradients estimators are unbiased, i.e. $\EE{S_2}{g_{S_2}(\theta)} = \nabla \Lcal_2(\theta)$. 
%
%We remind that the probability for an element $i$ to be in a set $S$ of $m$ elements sampled uniformly without replacement from $n$ elements satisfy
%\begin{equation}
%\mathbb{P}(i\in S)
%= \frac{m }{n}
%\text{ and }
%\mathbb{P}((i, j)\in S)
%= \frac{m }{n}\frac{m-1}{n-1}
%,
%\end{equation}
%
%\begin{equation}
%\sigma_x(\theta) \coloneqq \EE{S_x}{\norm{g_{S_x}(\theta)  - \nabla \Lcal_2(\theta)}^2}
%\end{equation}
%
%\subsection*{Method 1: Vanilla SGD}
%
%
%
%\begin{align}
%\sigma_1(\theta)
%&= \E{\norm{\sum_{i=1}^{n-1} (\omega_i(S_1) - \frac{1}{n-1}) \nabla l_i(\theta)}^2}
%\\
%%	&= \sum_{i=1}^{n-1}  \E{\left(\omega_i(S_1) - \frac{1}{n-1}\right)^2} \norm{\nabla l_i(\theta)}^2
%%	\nonumber\\
%%	&+ \sum_{i=1}^{n-1}\sum_{j \neq i} \E{(\omega_i(S_1) - \frac{1}{n-1}) (\omega_j(S_1) - \frac{1}{n-1}) } \nabla l_i(\theta)^T \nabla l_j(\theta)
%%	\\
%&= \sum_{i=1}^{n-1}  \VAR{\omega_i(S_1)} \norm{\nabla l_i(\theta)}^2
%+ \sum_{i=1}^{n-1}\sum_{j \neq i} \COV{\omega_i(S_1)}{\omega_j(S_1)} \nabla l_i(\theta)^T \nabla l_j(\theta)
%%	\\
%\label{eq:def_sigma1}
%\end{align}
%$m$ out of $n$ elements are sampled uniformly without replacement which gives
%\begin{align}
%\VAR{\omega_i(S_1)}
%&= \alpha_1 
%\coloneqq\frac{1}{n-1} \left[\frac{1}{m}- \frac{1}{n-1}\right]
%\\
%\COV{\omega_i(S_1)}{\omega_j(S_1)}
%&= - \frac{1}{(n-1)(n-2)}\left[\frac{1}{m}- \frac{1}{n-1}\right]
%= - \frac{1}{n-2}\alpha_1
%\label{eq:calculus_S1}
%\end{align}
%
%Substituting equation (\ref{eq:calculus_S1}) in equation (\ref{eq:def_sigma1}) gives
%\begin{equation}
%\sigma_1(\theta)
%= \sum_{i=1}^{n-1}  \alpha_1 \norm{\nabla l_i(\theta)}^2
%- \frac{1}{n-2}\alpha_1 \sum_{i=1}^{n-1}\sum_{j \neq i} \nabla l_i(\theta)^T \nabla l_j(\theta)
%\end{equation}
%
%We note that 
%\begin{equation}
%\sum_{i=1}^{n-1}\sum_{j \neq i} \nabla l_i(\theta)^T \nabla l_j(\theta)
%= 
%\norm{\sum_{i=1}^{n-1} \nabla l_i(\theta)}^2
%-
%\sum_{i=1}^{n-1} \norm{\nabla l_i(\theta)}^2
%\end{equation}
%which gives
%\begin{align}
%\sigma_1(\theta)
%&= \frac{n-1}{n-2} \alpha_1 \sum_{i=1}^{n-1}  \norm{\nabla l_i(\theta)}^2
%- \frac{1}{n-2}\alpha_1 \norm{\sum_{i=1}^{n-1}\nabla l_i(\theta)}^2 
%\\
%&= \frac{n-1}{n-2} \alpha_1 \sum_{i=1}^{n-1}  \norm{\nabla l_i(\theta)}^2
%- \frac{(n-1)^2}{n-2}\alpha_1 \norm{\nabla \Lcal_2(\theta)}^2 
%\end{align}
%Let us note that
%\begin{equation}
%	\norm{\nabla l_i(\theta)}^2
%	=
%	\norm{\nabla l_i(\theta) - \nabla \Lcal_2(\theta)}^2
%	+
%	\norm{\nabla \Lcal_2(\theta)}^2
%	+ 
%	2 \inner{\nabla l_i(\theta) - \nabla \Lcal_2(\theta)}{\nabla \Lcal_2(\theta)}
%\end{equation}
%which gives 
%\begin{equation}
%\sum_{i=1}^{n-1}\norm{\nabla l_i(\theta)}^2
%=
%\sum_{i=1}^{n-1} \norm{\nabla l_i(\theta) - \nabla \Lcal_2(\theta)}^2
%+
%\sum_{i=1}^{n-1} \norm{\nabla \Lcal_2(\theta)}^2
%\end{equation}
%and
%\begin{align}
%\sigma_1(\theta)
%&= \frac{n-1}{n-2} \alpha_1 \sum_{i=1}^{n-1}  \norm{\nabla l_i(\theta) - \nabla \Lcal_2(\theta)}^2
%- n \frac{n-1}{n-2}\alpha_1 \norm{\nabla \Lcal_2(\theta)}^2 
%\end{align}
%
%
%\subsection*{Method 2: Ours}
%
%\begin{align}
%\sigma_2(\theta)
%&=  \E{\norm{\sum_{i=1}^{n-1} \left(\omega_i(S_2) - \frac{1}{n-1}\right) \nabla l_i(\theta)
%		+ \left(\omega_n(S_2) + \omega_{n+1}(S_2)\right) \nabla l_n(\theta)}^2}
%\\
%&=  \E{\norm{\sum_{i=1}^{n-1} \left(\omega_i(S_2) - \frac{1}{n-1}\right) \nabla l_i(\theta)}^2}
%	+\E{\left(\omega_{n+1}(S_2) + \omega_{n+1}(S_2)\right)^2 }\norm{\nabla l_n(\theta)}^2
%\nonumber\\
%&+ 2  \sum_{i=1}^n \E{\left(\omega_i(S_2) - \frac{1}{n-1}\right)\left(\omega_{n+1}(S_2) + \omega_{n+1}(S_2)\right)}
%\nabla l_i(\theta)^T\nabla l_n(\theta)
%%\\
%%&= \sum_{i=1}^{n-1}  \VAR{\omega_i(S_1)} \norm{\nabla l_i(\theta)}^2
%%+ \sum_{i=1}^{n-1}\sum_{j \neq i} \COV{\omega_i(S_1)}{\omega_j(S_1)} \nabla l_i(\theta)^T \nabla l_j(\theta)
%%\\
%\label{eq:def_sigma2}
%\end{align}
%
%\begin{align}
%\VAR{\omega_i(S_2)}
%&
%= \alpha_2 
%\coloneqq \frac{n - m +1}{m(n-1)^2}
%\\
%\COV{\omega_i(S_2)}{\omega_j(S_2)}
%&
%= - \frac{n - m + 1}{ ( n - 1 )^2 n m }
%= - \frac{1}{n}\alpha_2
%\label{eq:calculus_S2_Var}
%\end{align}
%\begin{equation}
%	\E{\left(\omega_{n+1}(S_2) + \omega_{n+1}(S_2)\right)^2 }
%	= \E{\omega_{n+1}^2(S_2)} + \E{ \omega_{n+1}^2(S_2)} - \frac{2}{(n-1)^2}
%	= 2 \alpha_2
%\end{equation}
%
%Substituting equation (\ref{eq:calculus_S2_Var}) in equation (\ref{eq:def_sigma2}) and reproducing the same steps to obtain $\sigma_1(\theta)$ gives
%\begin{align}
%\sigma_2(\theta)
%&=  \sum_{i=1}^{n-1}  \alpha_2 \norm{\nabla l_i(\theta)}^2
%- \frac{1}{n}\alpha_2 \sum_{i=1}^{n-1}\sum_{j \neq i} \nabla l_i(\theta)^T \nabla l_j(\theta)
%+2\alpha_2\norm{\nabla l_n(\theta)}^2
%%\nonumber\\
%%&- 2 \frac{1}/{n} \alpha_2\sum_{i=1}^n 
%%\nabla l_i(\theta)^T\nabla l_n(\theta)
%\\
%&=  \left[ 1  + \frac{1}{n}\right] \alpha_2 \sum_{i=1}^{n-1}  \norm{\nabla l_i(\theta)}^2
%- \frac{ (n-1)^2  }{n}\alpha_2 \norm{\nabla \Lcal_2(\theta)}^2
%+2\alpha_2\norm{\nabla l_n(\theta)}^2
%\end{align}
%
%Similarly, we have
%\begin{align}
%\sigma_2(\theta)
%&=  \left[ 1  + \frac{1}{n}\right] \alpha_2 \sum_{i=1}^{n-1}  \norm{\nabla l_i(\theta) - \nabla \Lcal_2 (\theta)}^2
%- \alpha_2 (n-3) \norm{\nabla \Lcal_2(\theta)}^2
%+2\alpha_2\norm{\nabla \Lcal_1(\theta) - \nabla \Lcal_2(\theta)}^2
%\end{align}
%
%
%
%
%
%
%\subsection*{Comparison at beginning of unlearning}
%
%
%\begin{align}
%\sigma_1(\theta_1^*)
%&= \frac{n-1}{n-2} \alpha_1 \sum_{i=1}^{n-1}  \norm{ \nabla l_i(\theta_1^*) - \nabla \Lcal_2(\theta_1^*)}^2
%- n \frac{n-1}{n-2}\alpha_1 \norm{\nabla \Lcal_2(\theta_1^*)}^2 
%\end{align}
%
%
%\begin{align}
%\sigma_2(\theta_1^*)
%&=  \left[ 1  + \frac{1}{n}\right] \alpha_2 \sum_{i=1}^{n-1}  \norm{ \nabla l_i(\theta_1^*) - \nabla \Lcal_2(\theta_1^*)}^2
%- \alpha_2 (n-5)\norm{\nabla \Lcal_2(\theta_1^*)}^2
%\end{align}
%
%
%
%\subsection*{General}
%\begin{align}
%\sigma(\theta)
%&=  \E{\norm{\sum_{i=1}^{n-1} \left(\omega_i - \frac{1}{n-1}\right) \nabla l_i(\theta)
%		+ \left(\omega_n + \omega_{n+1}\right) \nabla l_n(\theta)}^2}
%\\
%&=  \E{\norm{\sum_{i=1}^{n-1} \left(\omega_i - \frac{1}{n-1}\right) \nabla l_i(\theta)}^2}
%+\E{\left(\omega_{n+1} + \omega_{n+1} \right)^2 }\norm{\nabla l_n(\theta)}^2
%\nonumber\\
%&+ 2  \sum_{i=1}^{n-1} \E{\left(\omega_i - \frac{1}{n-1}\right)\left(\omega_n + \omega_{n+1} \right)}
%\nabla l_i(\theta)^T\nabla l_n(\theta)
%\label{eq:def_sigmaG}
%\end{align}
%The third term is null. $m$ samples are selected with replacement with probability $p_i$. Hence, we have
%\begin{equation}
%	\omega_i = 
%	\begin{cases}
%	\frac{1}{n-1}\frac{1}{mp_i}\sum_{k=1}^m \mathbb{I}(l_k = i)
%	& \text{if } i \le n-1
%	\\
%	a_n \frac{1}{m}\sum_{k=1}^m \mathbb{I}(l_k = n)
%	& \text{if } i=n
%	\\
%	- a_{n+1} \frac{1}{m }\sum_{k=1}^m \mathbb{I}(l_k = n+1)
%	& \text{if } i=n+1
%	\end{cases}
%\end{equation}
%where the weights when $i\le n-1$ are assigned such that $\E{\omega_i} = \frac{1}{n-1}$ and $\E{\omega_n + \omega_{n+1}} = 0$. As such, we have $a_n p_n= a_{n+1} p_{n+1}$ which gives
%\begin{align}
%\VAR{\omega_i}
%&
%= \frac{1}{(n-1)^2}\frac{1}{mp_i}(1-p_i) 
%\\
%\COV{\omega_i}{\omega_j}
%&
%= - \frac{1}{(n-1)^2} \frac{m- 1}{m} 
%\\
%\E{\left(\omega_n + \omega_{n+1}\right)^2 }
%&= \E{\omega_n^2} 
%+ \E{ \omega_{n+1}^2} 
%+ 2 \E{ \omega_n \omega_{n+1} }
%\\
%&= \frac{1}{m}a_n^2 \left[p_n^2 (m-1) + p_n\right]
%+ \frac{1}{m}a_{n+1}^2 \left[p_{n+1}^2 (m-1) + p_{n+1}\right]
%- 2\frac{m-1}{m}a_n a_{n+1}p_n p_{n+1}
%\\
%&= \frac{m-1}{m}(a_n p_n - a_{n+1} p_{n+1})^2
%+ \frac{1}{m}a_n^2 p_n
%+ \frac{1}{m}a_{n+1}^2 p_{n+1}
%\\
%&= 
%\frac{1}{m}a_n^2 p_n
%+ \frac{1}{m}a_{n+1}^2 p_{n+1}
%\\
%\end{align}
%
%Substituting equation (\ref{eq:calculus_S2_Var}) in equation (\ref{eq:def_sigma2}) and reproducing the same steps to obtain $\sigma_1(\theta)$ gives
%\begin{align}
%\sigma(\theta)
%&=  \sum_{i=1}^{n-1}  \frac{1}{(n-1)^2}\frac{1}{mp_i}(1-p_i) \norm{\nabla l_i(\theta)}^2
%- \frac{1}{(n-1)^2} \frac{m- 1}{m}  \sum_{i=1}^{n-1}\sum_{j \neq i} \nabla l_i(\theta)^T \nabla l_j(\theta)
%\nonumber\\
%& +\beta(n) \norm{\nabla l_n(\theta)}^2
%\\
%&=  \frac{1}{m(n-1)^2}\sum_{i=1}^{n-1}  \left[\frac{1}{p_i} + m -2\right]\norm{\nabla l_i(\theta)}^2
%- \frac{m-1}{m}\norm{\nabla \Lcal_2(\theta)}^2
%+ \beta(n) \norm{\nabla l_n(\theta)}^2
%\\
%&=  \frac{1}{m(n-1)^2}\sum_{i=1}^{n-1}  \frac{1}{p_i} \norm{\nabla l_i(\theta)}^2
%+ \frac{m-2}{m}\sum_{i=1}^{n-1} \norm{ \frac{1}{n-1}\nabla l_i(\theta) - \nabla \Lcal_2(\theta)}^2
%\nonumber\\
%&
%- \frac{1}{m}\norm{\nabla \Lcal_2(\theta)}^2
%+ \beta(n) \norm{\nabla \Lcal_2(\theta) - \nabla \Lcal_1(\theta)}^2
%\end{align}
%
%When we do not consider the sample that has been deleted for retraining, we get $p_n = p_{n+1} = 0$ which gives:
%\begin{align}
%\sigma(\theta)
%&=  \frac{1}{m(n-1)^2}\sum_{i=1}^{n-1}  \frac{1}{p_i} \norm{\nabla l_i(\theta)}^2
%+ \frac{m-2}{m}\sum_{i=1}^{n-1} \norm{ \frac{1}{n-1}\nabla l_i(\theta) - \nabla \Lcal_2(\theta)}^2
%- \frac{1}{m}\norm{\nabla \Lcal_2(\theta)}^2
%,
%\end{align}
%which is minimized when the first term is minimized when $p_i$ satisfies
%\begin{equation}
%	p_i = \frac{\norm{\nabla l_i(\theta)}}{\sum_{i=1}^{n-1}\norm{\nabla l_i(\theta)}}
%\end{equation}
%In that case, we have
%\begin{align}
%\sigma(\theta)
%&=  \frac{1}{m(n-1)^2}\left[\sum_{i=1}^{n-1} \norm{\nabla l_i(\theta)}\right]^2
%+ \frac{m-2}{m}\sum_{i=1}^{n-1} \norm{ \frac{1}{n-1}\nabla l_i(\theta) - \nabla \Lcal_2(\theta)}^2
%- \frac{1}{m}\norm{\nabla \Lcal_2(\theta)}^2
%,
%\end{align}
%
%More generally,
%we have
%\begin{equation}
%p_i = ( 1 - p_n - p_{n+1})\frac{\norm{\nabla l_i(\theta)}}{\sum_{i=1}^{n-1}\norm{\nabla l_i(\theta)}}
%\end{equation}
%which gives
%\begin{align}
%\sigma(\theta)
%&=  \frac{1}{1 - p_n - p_{n+1}} \frac{1}{m(n-1)^2}\left[\sum_{i=1}^{n-1} \norm{\nabla l_i(\theta)}\right]^2
%+ \frac{m-2}{m}\sum_{i=1}^{n-1} \norm{ \frac{1}{n-1}\nabla l_i(\theta) - \nabla \Lcal_2(\theta)}^2
%\nonumber\\
%&- \frac{1}{m}\norm{\nabla \Lcal_2(\theta)}^2
%+ \beta(n) \norm{\nabla \Lcal_2(\theta) - \nabla \Lcal_1(\theta)}^2
%,
%\end{align}
%
%Therefore we have
%\begin{align}
%	&\sigma_2(\theta) - \sigma_1(\theta)
%	\nonumber\\
%	& = \left[\frac{1}{1 - p_n - p_{n+1}} - 1\right]\frac{1}{m(n-1)^2}\left[\sum_{i=1}^{n-1} \norm{\nabla l_i(\theta)}\right]^2
%	+ \beta(n) \norm{\nabla l_n(\theta)}^2
%\end{align}



























==> tex/application_FL.tex <==
When working with many clients where only some of the clients can be forgotten, a client can be split in many other clients. 


==> tex/application_centralized.tex <==
When working with too many clients,  clusters of clients can instead be created. As such, a set of clients is forgotten instead of just one. 

Extension to shards

==> tex/applications.tex <==
\section{Applications}\label{sec:applications}

\subsection{Centralized Learning}\label{subsec:centralized}
\input{./tex/application_centralized}


\subsection{DL and FL}\label{subsec:DL}
\input{./tex/application_FL}

==> tex/background.tex <==


\begin{definition}[DP]
	An Algorithm $\Acal$ satisfies ($\epsilon, \delta$)-differential privacy if for any two neighboring datasets $S$ and $S'$, differing in one sample, for any measurable event $E \in Range(\Acal)$,
	\begin{equation}
	\mathbb{P}(\Acal(S')\in E)
	\le e^\epsilon \mathbb{P}(\Acal(S)\in E)
	+ \delta
	\end{equation}
	
\end{definition}

\begin{definition}[indistinguishably]
	We say that $\Rcal_\Acal$ is an ($\epsilon$, $\delta$)-unlearning algorithm for $\Acal$ if for any two datasets $S$ and $S'$, differing in one sample, for any measurable event $E \in Range(\Acal)$, we have $\Rcal_\Acal(S) \indistin \Acal(S')$ defined as
	\begin{equation}
	\mathbb{P}(\Acal(S')\in E)
	\le e^\epsilon \mathbb{P}(\Acal(S)\in E)
	+ \delta
	,\
	\mathbb{P}(\Acal(S)\in E)
	\le e^\epsilon \mathbb{P}(\Acal(S')\in E)
	+ \delta
	.
	\end{equation}
	
\end{definition}


\begin{definition}
	A pair of $(\Acal, \Rcal_\Acal)$ learning and unlearning algorithms is ($\alpha$, $\beta$)-accurate 
	if for any two datasets $S$ and $S'$, differing in one sample, the following condition holds 
	\begin{equation}
		\mathbb{P}\left[\right]
	\end{equation}
\end{definition}


==> tex/convergence.tex <==
We use the dataset with all the data samples to unlearn data point $n$. 
$m$ samples are selected with replacement to create a batch. We consider $\mathbb{I}(l_k = i)$ the event that client $i$ is selected at $k$th position. We consider that client $n$ can either be drawn for gradient descent ($l_k = n$ ) or gradient ascent ($l_k = n+1$). We denote by $\omega_i$ the random variable associated to the weight of sample $i$. We consider that  $\mathbb{P}(l_k = i) = p_i$. Therefore, we have
\begin{equation}
\omega_i = 
\begin{cases}
\frac{1}{n-1}\frac{1}{mp_i}\sum_{k=1}^m \mathbb{I}(l_k = i)
& \text{if } i \le n-1
\\
a_n \frac{1}{n-1}\frac{1}{m}\sum_{k=1}^m \mathbb{I}(l_k = n)
& \text{if } i=n
\\
- a_{n+1} \frac{1}{n-1}\frac{1}{m }\sum_{k=1}^m \mathbb{I}(l_k = n+1)
& \text{if } i=n+1
\end{cases}
,
\end{equation}
where $a_n$ and $a_{n+1}$ are positive constants. We note that the samples kept in the dataset are in expectation properly sampled, i.e. $\E{\omega_i} = 1/(n-1)$. 

Let us call $g$ the gradient estimator of $\Lcal_2$. We have
\begin{equation}
g(\theta)
= \sum_{i=1}^{n-1} \omega_i \nabla l_i(\theta)
+ \left(\omega_n  + \omega_{n+1} \right) \nabla l_n(\theta)
.
\end{equation}
A sufficient condition for $g$ to be an unbiased gradient estimator is to have $\E{\omega_n  + \omega_{n+1}} =0$ which gives us $a_n p_n - a_{n+1} p_{n+1} = 0$. This shows the limit of an unbiased gradient estimator. Indeed, the deleted sample can only be considered for ascent if the sample can also be considered for descent and the other way around. As a result, the gradient estimator variance is higher by enabling sampling of deleted data samples with biased gradient estimators.
Therefore, we consider biased gradient estimators to get rid of this last inequality between $p_n$ and $p_{n+1}$.


\subsection{Theoretical Work}

$\EE{S}{X}$ is the expected value of $X$ over $S$ the random set of sampled clients.
If we consider the Lipschitz smoothness of $f$, we get
\begin{equation}
	\EE{S}{f(x^{t+1}) - f(x^{t})}
	\le - \gamma \EE{S}{\inner{\nabla f(x^t)}{g(x^t)}}
	+ \frac{L}{2}\gamma \EE{S}{\norm{g_t}^2}
	\label{app:eq:A0}
\end{equation}
%
%\begin{equation}
%\omega_i = 
%\begin{cases}
%\frac{1}{n-1}\frac{1}{mp_i}\sum_{k=1}^m \mathbb{I}(l_k = i)
%& \text{if } i \le n-1
%\\
%a_n \frac{1}{n-1}\frac{1}{m}\sum_{k=1}^m \mathbb{I}(l_k = n)
%& \text{if } i=n
%\\
%- a_{n+1} \frac{1}{n-1}\frac{1}{m }\sum_{k=1}^m \mathbb{I}(l_k = n+1)
%& \text{if } i=n+1
%\end{cases}
%\end{equation}

\subsubsection*{1st term}
We define $\alpha(n) \coloneqq a_n p_n - a_{n+1} p_{n+1}$ which gives
\begin{equation}
	\EE{S}{g(x^t)}
	= \nabla f ( x^t) 
	+ \frac{1}{n-1} \frac{1}{m} \alpha(n) \nabla l_n(x^t)
	,
\end{equation}
and
\begin{equation}
\inner{\nabla f(x^t)}{\EE{S}{g(x^t)}}
= \norm{\nabla f ( x^t)}^2 
+ \frac{1}{n-1}\frac{1}{m} \alpha(n)
%\left[a_n p_n - a_{n+1} p_{n+1} \right]
\inner{\nabla f(x^t)}{\nabla l_n(x^t)}
\label{app:eq:A1}
,
\end{equation}

\subsubsection*{2nd term}
Considering 
\begin{align}
\E{\omega_i^2}
&
= \frac{1}{(n-1)^2} \left[\frac{m-1}{m} + \frac{1}{mp_i}\right] 
\\
\E{\omega_i\omega_j}
&
= \frac{1}{(n-1)^2} \frac{m- 1}{m} 
\\
\E{\left(\omega_n + \omega_{n+1}\right)^2 }
&= \E{\omega_n^2} 
+ \E{ \omega_{n+1}^2} 
+ 2 \E{ \omega_n \omega_{n+1} }
\\
&= \frac{1}{(n-1)^2}
\left[\frac{m-1}{m}\alpha^2(n)
+ \frac{1}{m}a_n^2 p_n
+ \frac{1}{m}a_{n+1}^2 p_{n+1}\right]
\eqqcolon \beta(n)
,
\end{align}
we get
\begin{align}
\EE{S}{\norm{g_t}^2}
& = \sum_{i =1}^{n-1} \sum_{ j = 1 }^{ n - 1 } \E{\omega_i \omega_j} \nabla l_i(x^t)^T \nabla l_j(x^t)
+ \E{(\omega_n + \omega_{n+1})^2} \norm{\nabla l_n(x^t)}^2
\nonumber\\
& + 2 \sum_{i =1}^{n-1} \E{\omega_i (\omega_n + \omega_{n+1})} \nabla l_i(x^t)^T \nabla l_n(x^t)
\\
& = \frac{1}{(n-1)^2}\frac{1}{m}\sum_{i =1}^{n-1} \frac{1}{p_i} \norm{\nabla l_i(x^t)}^2
+ \frac{m-1}{m} \norm{\nabla f(x^t)}^2
+ \beta(n) \norm{\nabla l_n(x^t)}^2
\nonumber\\
& + 2 \frac{1}{(n-1)^2}\frac{m-1}{m}\alpha(n)\nabla f(x^t)^T \nabla l_n(x^t)
\label{app:eq:A2}
,
\end{align}

\subsubsection*{Rewrite inner product}
We can rewrite the gradient of the previous loss function as 
\begin{equation}
	\nabla \Lcal_1(x^t)
	= \frac{n-1}{n}\nabla f(x^t)
	+ \frac{1}{n}\nabla l_n(x^t)
	,
\end{equation}
which gives
\begin{align}
	\inner{\nabla f(x^t)}{\nabla l_n(x^t)}
	& = \frac{n^2}{n-1} \inner{\frac{n-1}{n}\nabla f(x^t)}{\frac{1}{n}\nabla l_n(x^t)}
	\\
	& = \frac{n^2}{n-1} \frac{1}{2} \left[ \norm{\nabla \Lcal_1(x^t)}^2 
	-\frac{(n-1)^2}{n^2}\norm{\nabla f(x^t)}^2
	-\frac{1}{n^2}\norm{\nabla l_n(x^t)}^2
	\right]
\end{align}
%\begin{align}
%\inner{\nabla f(x^t)}{\EE{S}{g(x^t)}}
%& = \left[1 - \frac{n-1}{2}\frac{1}{m} \alpha(n)\right]\norm{\nabla f ( x^t)}^2 
%\nonumber\\
%& + \frac{n^2}{2(n-1)} \frac{1}{m} \alpha(n) \norm{\nabla \Lcal_1(x^t)}^2
%- \frac{1}{2(n-1)} \frac{1}{m} \alpha(n) \norm{\nabla l_n(x^t)}^2
%,
%\end{align}

\subsubsection*{Merge}
Substituting equation (\ref{app:eq:A1}) and (\ref{app:eq:A2}) in (\ref{app:eq:A0}) gives
\begin{align}
\frac{1}{\gamma}\E{f(x^{t+1}) - f(x^{t})}
&\le - \left[1 - \frac{L}{2}\gamma \frac{m-1}{m}\right] \norm{\nabla f(x^t)}^2
\nonumber\\
&- \left[1 - L\gamma \frac{m-1}{m}\right] 
\frac{1}{n-1}\frac{1}{m}\alpha(n) \nabla f(x^t)^T \nabla l_n(x^t) 
\nonumber\\
&+ \frac{L}{2} \gamma  \frac{1}{(n-1)^2} \frac{1}{m} \sum_{i =1}^{n-1} \frac{1}{p_i}\norm{\nabla l_i(x^t)}^2
+ \frac{L}{2}\gamma \beta(n) \norm{\nabla l_n(x^t)}^2
.
\label{app:eq:B1}
\end{align}
We note at this point that the only influence of $p_i$ lies in $\sum_{i =1}^{n-1}\frac{1}{p_i}\norm{\nabla l_i(x^t)}^2$ which for all $p_n$ and $p_{n+1}$ is minimized when 
\begin{equation}
p_i = (1 - p_n - p_{n+1})\frac{\norm{\nabla l_i(\theta)}}{\sum_{i=1}^{n-1}\norm{\nabla l_i(\theta)}}
.
\end{equation}
Therefore equation (\ref{app:eq:B1}) cn be simplified as
\begin{align}
\frac{1}{\gamma}\E{f(x^{t+1}) - f(x^{t})}
&\le - \left[1 - \frac{L}{2}\gamma \frac{m-1}{m}\right] \norm{\nabla f(x^t)}^2
\nonumber\\
&- \left[1 - L\gamma \frac{m-1}{m}\right] 
\frac{1}{n-1}\frac{1}{m}\alpha(n) \nabla f(x^t)^T \nabla l_n(x^t) 
\nonumber\\
&+ \frac{L}{2} \gamma  \frac{1}{(n-1)^2} \frac{1}{m} \frac{1}{1 - p_n - p_{n+1}} \left[\sum_{i =1}^{n-1} \norm{\nabla l_i(x^t)}\right]^2
+ \frac{L}{2}\gamma \beta(n) \norm{\nabla l_n(x^t)}^2
.
\label{app:eq:B2}
\end{align}
In the rest of this work, we assume that $1 - L\gamma \frac{m-1}{m}>0$.
For the biased gradient estimator to provide a faster convergence process, the deleted sample needs to be considered for descent or ascent such that $\alpha(n) \nabla f(x^t)^T \nabla l_n(x^t) \ge 0 $ is satisfied which can be rewritten as
\begin{align}
	&\alpha(n) \inner{ \nabla f(x^t)^T }{\nabla l_n(x^t) }
	\nonumber\\	
	&\alpha(n) \frac{n^2}{n-1}\inner{\frac{n-1}{n}\nabla f(x^t)^T }{\frac{1}{n}\nabla l_n(x^t) }
	\\
	&=
	\alpha(n) \frac{n^2}{n-1}
	\left[ \norm{\nabla \Lcal_1(x^t)}^2 - \left[\frac{n-1}{n}\right]^2\norm{\nabla f(x^t)}^2  - \frac{1}{n^2}\norm{\nabla l_n(x^t)}^2 \right]
	\ge 0
\end{align}
We are interested in improving the unlearning process. Especially to leave faster the initial model $\theta_1^*$. for which, we have $\nabla \Lcal_1(\theta_1^*)= 0$. Therefore, regardless of whether a deleted sample is considered to obtain the biased gradient estimator, we have $p_n =0$. Therefore $\alpha(n) = - a_{n+1} p_{n+1}$ and $\beta(n) = \frac{1}{(n-1)^2}\left[\frac{m-1}{m}a_{n+1}^2 p_{n+1}^2 + \frac{1}{m}a_{n+1}^2 p_{n+1} \right]$. We obtain
\begin{align}
\frac{1}{\gamma}\E{f(x^{t+1}) - f(x^{t})}
&\le - \left[\left[1 - \frac{L}{2}\gamma \frac{m-1}{m}\right] + \left[1 - L\gamma \frac{m-1}{m}\right] \frac{1}{m} a_{n+1}p_{n+1} \right] \norm{\nabla f(x^t)}^2
\nonumber\\
&- \left[1 - L\gamma \frac{m-1}{m}\right] 
\frac{n^2}{(n-1)^2}\frac{1}{m} a_{n+1}p_{n+1} \norm{\nabla \Lcal_1(x^t) }^2
\nonumber\\
&+ \frac{L}{2} \gamma  \frac{1}{(n-1)^2} \frac{1}{m} \frac{1}{1 - p_{n+1}} \left[\sum_{i =1}^{n-1} \norm{\nabla l_i(x^t)}\right]^2
\nonumber\\
&+ \left[\frac{L}{2}\gamma \beta(n) + \left[1 - L\gamma \frac{m-1}{m}\right] 
\frac{1}{(n-1)^2}\frac{1}{m} a_{n+1}p_{n+1}\right]\norm{\nabla l_n(x^t)}^2
.
\label{app:eq:B3}
\end{align}

\begin{align}
\frac{1}{\gamma}\E{f(x^{t+1}) - f(x^{t})}
&\le - \left[1 + \frac{1}{m} a_{n+1}p_{n+1} \right] \norm{\nabla f(x^t)}^2
- \frac{n^2}{(n-1)^2}\frac{1}{m} a_{n+1}p_{n+1} \norm{\nabla \Lcal_1(x^t) }^2
\nonumber\\
&+ \frac{L}{2} \gamma  \frac{1}{(n-1)^2} \frac{1}{m} \frac{1}{1 - p_{n+1}} \left[\sum_{i =1}^{n-1} \norm{\nabla l_i(x^t)}\right]^2
\nonumber\\
&+ \left[\frac{L}{2}\gamma \beta(n) +  
\frac{1}{(n-1)^2}\frac{1}{m} a_{n+1}p_{n+1}\right]\norm{\nabla l_n(x^t)}^2
.
\label{app:eq:B4}
\end{align}

We also define
\begin{equation}
	A(t)
	= \frac{1}{\gamma}\E{f(x^{t}) - f(x^{t+1})}
	,\
	B(t)
	= \left[1 - L\gamma \frac{m-1}{m}\right] 
	\frac{1}{n-1}\frac{1}{m} \nabla f(x^t)^T \nabla l_n(x^t)
\end{equation}
\begin{equation}
	C(t)
	= \frac{L}{2} \gamma  \frac{1}{(n-1)^2} \frac{1}{m} \left[\sum_{i =1}^{n-1} \norm{\nabla l_i(x^t)}\right]^2
	,\
	D(t)
	= \frac{L}{2}\gamma \frac{1}{(n-1)^2} \frac{m-1}{m}\norm{\nabla l_n(x^t)}^2
\end{equation}
\begin{equation}
	E(t)
	= \frac{L}{2}\gamma \frac{1}{(n-1)^2} \frac{1}{m}\norm{\nabla l_n(x^t)}^2
\end{equation}


 which gives
\begin{align}
\left[1 - \frac{L}{2}\gamma \frac{m-1}{m}\right] \norm{\nabla f(x^t)}^2
&\le A(t) - B(t) a_{n+1} p_{n+1}
\nonumber\\
&+ \frac{1}{1 - p_{n+1}} C(t) 
+ D(t) a_{n+1}^2 p_{n+1}^2 
+ E(t) a_{n+1}^2 p_{n+1} 
.
\label{app:eq:B3}
\end{align}
We consider the loss function where we replace $\frac{1}{1-p_{n+1}} =  1 + p_{n+1} + p_{n+1}^2$.
Let us consider
\begin{equation}
	f(x^t)
	= \left[ - B(t) a_{n+1}+ C(t) + E(t) a_{n+1}^2\right]p_{n+1}
	+ \left[ C(t) + D(t) a_{n+1}^2\right] p_{n+1}^2 
\end{equation}
We therefore have
\begin{equation}
	content...
\end{equation}




\subsubsection*{Not Kept}
\begin{align}
\frac{1}{\gamma}\E{f(x^{t+1}) - f(x^{t})}
&\le - \rho \left[1 - \frac{1}{2}\frac{1}{m}\alpha(n)\right]\norm{\nabla f(x^t)}^2
- \rho \alpha(n) \frac{1}{2} \frac{n^2}{(n-1)^2} \frac{1}{m}\norm{\nabla \Lcal_1(x^t)}^2 
\nonumber\\
&+ \frac{L}{2}\gamma\frac{1}{m}\frac{1}{(n-1)^2} \sum_{i =1}^{n-1} \frac{1}{p_i}\norm{\nabla l_i(x^t)}^2
\nonumber\\
&+ \frac{1}{(n-1)^2}\left[\frac{1}{2}\frac{1}{m}\alpha(n)\rho + \frac{L}{2}\gamma \beta'(n) \right] \norm{\nabla l_n(x^t)}^2
\end{align}

We note that the importance $p_i$ given to each sample $i \le n$ can already be allocated such that 
\begin{equation}
p_i = (1 - p_n - p_{n+1})\frac{\norm{\nabla l_i(\theta)}}{\sum_{i=1}^{n-1}\norm{\nabla l_i(\theta)}}
\end{equation}

Lastly, the bound is proportional to $p_n$ and $p_{n+1}$. Therefore, only $p_n$ or $p_{n+1}$ is positive. 

If we consider that we are at the optimum, one gets
\begin{equation}
\nabla \Lcal_1(x_1^*) 
= \frac{n-1}{n}\nabla f(x_1^*)
+ \frac{1}{n}\nabla l_n(x_1^*)
=0
,
\end{equation}
\begin{align}
\frac{1}{\gamma}\E{f(x^{t+1}) - f(x^{t})}
&\le - \left[ \rho \left[ 1
- \frac{1}{m}\alpha(n)  \right] 
- \frac{L}{2}\gamma \beta'(n)\right]
\norm{\nabla f(x_1^*)}^2
\nonumber\\
&+ \frac{L}{2}\gamma\frac{1}{m}\frac{1}{(n-1)^2} \frac{1}{1- p_n - p_{n+1}}\left[\sum_{i =1}^{n-1} \norm{\nabla l_i(x_1^*)}\right]^2
\end{align}




where the weights when $i\le n-1$ are assigned such that $\E{\omega_i} = \frac{1}{n-1}$ and $\E{\omega_n + \omega_{n+1}} = 0$. As such, we have $a_n p_n= a_{n+1} p_{n+1}$ which gives
\begin{align}
\VAR{\omega_i}
&
= \frac{1}{(n-1)^2}\frac{1}{mp_i}(1-p_i) 
\\
\COV{\omega_i}{\omega_j}
&
= - \frac{1}{(n-1)^2} \frac{m- 1}{m} 
\\
\E{\left(\omega_n + \omega_{n+1}\right)^2 }
&= \E{\omega_n^2} 
+ \E{ \omega_{n+1}^2} 
+ 2 \E{ \omega_n \omega_{n+1} }
\\
&= \frac{1}{m}a_n^2 \left[p_n^2 (m-1) + p_n\right]
+ \frac{1}{m}a_{n+1}^2 \left[p_{n+1}^2 (m-1) + p_{n+1}\right]
- 2\frac{m-1}{m}a_n a_{n+1}p_n p_{n+1}
\\
&= \frac{m-1}{m}(a_n p_n - a_{n+1} p_{n+1})^2
+ \frac{1}{m}a_n^2 p_n
+ \frac{1}{m}a_{n+1}^2 p_{n+1}
\\
&= 
\frac{1}{m}a_n^2 p_n
+ \frac{1}{m}a_{n+1}^2 p_{n+1}
\\
\end{align}



In that case, we have
\begin{align}
\sigma(\theta)
&=  \frac{1}{m(n-1)^2}\left[\sum_{i=1}^{n-1} \norm{\nabla l_i(\theta)}\right]^2
+ \frac{m-2}{m}\sum_{i=1}^{n-1} \norm{ \frac{1}{n-1}\nabla l_i(\theta) - \nabla \Lcal_2(\theta)}^2
- \frac{1}{m}\norm{\nabla \Lcal_2(\theta)}^2
,
\end{align}

More generally,
we have
\begin{equation}
p_i = ( 1 - p_n - p_{n+1})\frac{\norm{\nabla l_i(\theta)}}{\sum_{i=1}^{n-1}\norm{\nabla l_i(\theta)}}
\end{equation}
which gives
\begin{align}
\sigma(\theta)
&=  \frac{1}{1 - p_n - p_{n+1}} \frac{1}{m(n-1)^2}\left[\sum_{i=1}^{n-1} \norm{\nabla l_i(\theta)}\right]^2
+ \frac{m-2}{m}\sum_{i=1}^{n-1} \norm{ \frac{1}{n-1}\nabla l_i(\theta) - \nabla \Lcal_2(\theta)}^2
\nonumber\\
&- \frac{1}{m}\norm{\nabla \Lcal_2(\theta)}^2
+ \beta(n) \norm{\nabla \Lcal_2(\theta) - \nabla \Lcal_1(\theta)}^2
,
\end{align}

Therefore we have
\begin{align}
	&\sigma_2(\theta) - \sigma_1(\theta)
	\nonumber\\
	& = \left[\frac{1}{1 - p_n - p_{n+1}} - 1\right]\frac{1}{m(n-1)^2}\left[\sum_{i=1}^{n-1} \norm{\nabla l_i(\theta)}\right]^2
	+ \beta(n) \norm{\nabla l_n(\theta)}^2
\end{align}



























==> tex/corollary.tex <==
%The proof of Theorem \ref{theo:diff_bound} (Appendix \ref{app:sec:proof_diff}) relies on deriving a lower bound for the Hessian of each client's loss function. This derivation however would require the server to obtain an estimate of the eigenvalues of each client's Hessian, which is generally not feasible in FL. 
Theorem \ref{theo:diff_bound} provides a bound for the model sensitivity quantified by the \emph{bounded sensitivity}, while the computation of (\ref{eq:def_Psi}) only requires the clients' updated models, which are already shared with the server by design in \textsc{FedAvg}. Nevertheless, we note that the bounded sensitivity (\ref{eq:def_Psi}) does not necessarily faithfully represent the evolution of the sensitivity across FL rounds. For instance, this quantity does not properly account for the unlearning of previous clients contributions  for $ s < n - 1 $. Indeed, these contributions should decrease across iterations due to the subsequent server aggregations and new clients' SGD steps.
To account for this aspect, we provide a tighter lower bound by assuming strongly convex and regularized local loss function, leading to a tighter bound for the model sensitivity of \textsc{FedAvg}  (Corollary \ref{cor:tighter}).

\begin{corollary}\label{cor:tighter}
	Under Assumption \ref{ass:linear_approx}, when considering that clients loss functions are $\mu$-strongly convex and regularized with an L2 norm of weight $\lambda$, we have $\alpha(n , c)\le \Psi(n , c)$ and
	\begin{equation}
	\Psi(n, c)
	= \sum_{s=0}^{n-1}\left(1 - \eta (\lambda + \mu )\right)^{\left[(n-1)-s\right]K} 
	\norm{\Delta(I, \vtheta^s) - \Delta(I_{-c}, \vtheta^s)}_2
	,
	\end{equation}
	where $\eta$ and $K$ are respectively the clients' local learning rate and amount of SGD steps.
\end{corollary}
\begin{proof}
	See Appendix \ref{app:subsec:regularization}.
\end{proof}

The bounded sensitivity of Corollary \ref{cor:tighter} shows the following aspects. (1) The importance of a client's contribution decreases through aggregation rounds.  
(2) Since FL is guaranteed to converge to a stationary point \cite{FedNova,OnTheConvergence}, so does the bounded sensitivity since $\lambda + \mu>0$.
(3) The bounded sensitivity is not necessarily inversely proportional to $K$. Indeed, due to data heterogeneity, with an increase in $K$ every  local model gets closer to its local optimum and the quantity $\norm{\Delta(I, \vtheta^n) - \Delta(I_{-c}, \vtheta^n)}_2$ increases with the amount of SGD steps $K$. 

When clients have same data distribution, we retrieve $\Delta(I, \vtheta^n) = \Delta(I_{-c}, \vtheta^n)$, which yields null bounded sensitivity for every client, i.e. $\Psi(n , c) = 0$. We also note that the bound provided in Corollary \ref{cor:tighter} is tight, e.g. when considering identical eigenvalues for the Hessian of every local loss. More generally, the bound is tight in the limit case where the local learning rate of the clients is small. 

We can draw an analogy between the bounded sensitivity (\ref{eq:def_Psi}) and client clustering in FL \cite{ClusteredFL,ClusteredSampling}, where clients are clustered based on their contribution. In this work, the bounded sensitivity (\ref{eq:def_Psi}) is used instead to bound the sensitivity of the global model across rounds in \textsc{FedAvg}.

==> tex/expansion.tex <==
\subsection*{Expansion}

Let us consider $\theta$ the model obtained by training with algorithm $\Acal$, and the perturbation $\delta$ brought to $S$, the resulting trained model is
\begin{equation}
	\Acal(S + \delta)
	= \Acal(S)
	+ \delta \nabla \Acal(S)
\end{equation}

$\delta_i$ is the modification of sampled $i$ and $S_i=(X_i, y_i)$ is sample $i$. We define $u$ the set of samples to forget. We consider there are $K$ classes. We define 
\begin{equation}
	\delta_i = 
	\begin{cases}
	\EE{X \sim X_i | y_i =y_k, i \in S'}{X} - X_k
	& \text{if } k\in u\\
	0
	& \text{otherwise}
	\end{cases}
\end{equation}

==> tex/figure_gradients.tex <==



\def\s{1.5} %space between columns
\def\h{-5} %height of columns
\def\id{0} %inner sep default
\def\i{7} %inner sep

\begin{figure}
	\begin{center}
	\begin{tikzpicture}[scale = 1, line cap=round, line join=round, >=triangle 45, x=1cm, y=1cm]
		
		

		%Beginnings/Ends
		\node[label=above: $\vtheta_0^0$, inner sep = \id] (A0) at (0,0){} ;
		\node[label=below: $\vtheta_0^{N_0}$, inner sep = \id] (Z0) at (0,\h){} ;
		
		\node[label= center: $\vtheta_1^0$, inner sep = \i] (A1) at ( \s, 2 * \h/5){} ;
		\node[label=below: $\vtheta_1^{N_1}$, inner sep = \id] (Z1) at (\s, \h){} ;
		
		\node[label= center: $\vtheta_2^0$, inner sep = \i] (A2) at ( 2 *\s, 3 * \h/5){} ;
		\node[label=below: $\vtheta_2^{N_2}$, inner sep = \id] (Z2) at (2 * \s, \h){} ;
		
		\node[label= center: $\vtheta_3^0$, inner sep = \i] (A3) at ( 3 *\s, \h/5){} ;
		\node[label=below: $\vtheta_3^{N_3}$, inner sep = \id] (Z3) at (3 * \s, \h){} ;
		
		\node[label= center: $\vtheta_4^0$, inner sep = \i] (A4) at ( 4 *\s, 2.5 * \h/5){} ;
		\node[label=below: $\vtheta_4^{N_4}$, inner sep = \id] (Z4) at (4 * \s, \h){} ;
		
		
		% Intermediary Points
		\node[inner sep = \id] (B0) at (0, \h/5){} ;
		\node[inner sep = \id] (C0) at (0, 2*\h /5){} ;
		
		\node[inner sep = \id] (B1) at (\s,  3 *\h/5){} ;
		
		\node[inner sep = \id] (B3) at (3 * \s,  2.5 *\h/5){} ;
		
		
		%Vertical Arrows
		\draw [line width=0.5pt, ->] (A0)-- (Z0);
		\draw [line width=0.5pt, ->] (A1)-- (Z1);
		\draw [line width=0.5pt, ->] (A2)-- (Z2);
		\draw [line width=0.5pt, ->] (A3)-- (Z3);
		\draw [line width=0.5pt, ->] (A4)-- (Z4);
		
		%Horizontal Arrows
		\draw [line width=0.5pt, ->] (C0) -- node[midway, above, align=center] {$\vtheta_0^{T_1}$} (A1) ;
		\draw [line width=0.5pt, ->] (B1) -- node[midway, above, align=center] {$\vtheta_1^{T_2}$} (A2) ;
		\draw [line width=0.5pt, ->] (B0) -- node[midway, above, align=center] {$\vtheta_{\zeta_3}^{T_3} = \vtheta_0^{T_3}$} (A3) ;
		\draw [line width=0.5pt, ->] (B3) -- node[midway, above, align=center] {$\vtheta_3^{T_4}$} (A4) ;
		
		
		%Horizontal Arrows
		\node[inner sep = \id] (AA) at (-0.2, \h - 1){} ;
		\node[label=below: 0, inner sep = \id] (BB) at (0, \h - 1){} ;
		\node[label=below: 1, inner sep = \id] (CC) at (\s, \h - 1){} ;
		\node[label=below: 2, inner sep = \id] (DD) at (2 * \s, \h - 1){} ;
		\node[label=below: 3, inner sep = \id] (EE) at (3 * \s, \h - 1){} ;
		\node[label=below: 4, inner sep = \id] (FF) at (4 * \s , \h - 1){} ;
		\node[label=below: $r$, inner sep = \id] (ZZ) at (4.5 * \s, \h - 1){} ;
		\draw [line width=0.5pt, ->] (AA)-- (ZZ);
		
	\end{tikzpicture}

	\end{center}
	
	\caption{An example of the flow of global models for four consecutive forgetting requests. }
	\label{fig:schematic_sim}
\end{figure}











==> tex/hessian_based.tex <==
\section{Formalizing the Unlearning problem}

\subsection{Optimization}
We consider a dataset $\Dcal$ composed of $|\Dcal| = N$ data samples $(\vx_i, \vy_i)$ where $\vx_i$ is the feature vector of a data sample and $\vy_i$ its prediction or label.
For unsupervised learning, it suffices to consider that data samples in $\Dcal$ are only made with $\vx_i$. We denote by $\Scal$ the set of $S = |\Scal|$ indices we want to forget from $\Dcal$ and $\Dcal_{-\Scal} = \Dcal\backslash\{(\vx_i, \vy_i) | i \in \Scal \}$ the dataset without the forgotten data samples.

We consider a function $f$ depending on one data sample and model parameters $\vtheta$. 
For example, $f$ can be the loss of one data sample or its activation vector. We define the associated normalized functions 
\begin{equation}
F(\vtheta) \coloneqq \frac{1}{|\Dcal|} \sum_{i \in \Dcal} f(\vx_i, \vy_i, \vtheta)
\text{ and }
F_{-\Scal}(\vtheta) \coloneqq \frac{1}{|\Dcal_{-\Scal}|} \sum_{i \in \Dcal_{-\Scal}} f(\vx_i, \vy_i, \vtheta)
.
\end{equation}
We consider $F$ is a $K$ dimensional vector where $K=1$ if $f$ is the loss function of one data samples and $K$ is the amount of classes in a classification problem. 
For ease of writing, we consider $F_{-i}$ to be the resulting function when forgetting data sample $i$. 


%\subsection{$(\epsilon, \delta)$-indistinguishable}
%
%%We first define $(\epsilon, \delta)$-indistinguishable in Definition \ref{def:DP_forget}.
%%\begin{definition}[$(\epsilon, \delta)$-indistinguishable] Let $\epsilon$ and $\delta$ be two positive real numbers. Two distributions $X$ and $Y$ are $(\epsilon, \delta)$-indistinguishable if for all subset $A \subseteq \Acal$, we have
%%	\label{def:DP_forget}
%%	\begin{equation}
%%	\mathbb{P}(X \in A) 
%%	\le e^\epsilon \mathbb{P}(Y \in A)  + \delta
%%	\text{ and }
%%	\mathbb{P}(Y \in A) 
%%	\le e^\epsilon \mathbb{P}(X \in A)  + \delta
%%	.
%%	\end{equation}
%%\end{definition}
%$\vtheta$ is the $d$ dimensional vector of the trained model parameters. We consider a stochastic perturbation $\vphi \sim N( \vmu, \mSigma)$, where $\mSigma$ is positive definite and can thus be expressed as $\mSigma = \mS^T \mS$, such that $F(\vtheta + \vphi)$ and $F_{-\Scal}(\vtheta + \vphi)$ are $(\epsilon, \delta)$-indistinguishable.
%
%Definition \ref{def:DP_forget} is linked to differential privacy(DP). With DP, we are looking at the noise $\vphi$ such that for any sample $i$, $F(\vtheta + \vphi)$ and $F_{-i}(\vtheta + \vphi)$ 
%are $(\epsilon, \delta)$-indistinguishable. In that case, no information specific to any data sample can be retrieve from $\hat{\vtheta} \coloneqq \vtheta + \vphi$. With Machine Unlearning, we are instead looking at $\vphi$ such that $\hat{\vtheta}$ does not contain specific information from any forgotten data sample. As such, DP implies Unlearning but Unlearning is weaker than DP.
%
%\begin{definition}[$(\epsilon, \delta, \Scal)$-unlearning] 
%	If $F(\vtheta + \vphi)$ and $F_{-\Scal}(\vtheta + \vphi)$ are $(\epsilon, \delta)$-indistinguishable, $\hat{\vtheta} \coloneqq \vtheta+ \vphi$ contains no information from $\Scal$.
%\end{definition}


\section{Scrubbing Methods}

We consider a quadratic approximation of every sample loss function.
Therefore, the scrubbing method $h$ satisfies 
\begin{equation}
	h(w) = w - H_w^{-1} \nabla f_{\Scal}(w)
\end{equation}



We can also analyze this transformation in function of the samples features on the scrubbed model

\begin{equation}
t(x_i) = x_i - H_x^{-1}(x_i, h(w)) \nabla_{x} f(x_i, h(w))
\end{equation}


The learnt model is not necessarily the best model to start the new learning process. 
We can bound the distance between a given model $w^t$ and the optimum model $w^*$ as :
We consider $H$ to be symmetric positive definite matrix.
\begin{align}
	\norm{w^t - w^*}_2^2
	&= \norm{w^t - h(w^t)}_2^2
	= \norm{H^{-1}\nabla f}_2^2
	\le \norm{H^{-1}}_F^2 \norm{\nabla f}_2^2
	\\
	&= \Tr{\left(H^{-2}\right)} \norm{\nabla f}_2^2
	\le \Tr{\left(H\right)}^{-2} \norm{\nabla f}_2^2
	= \left(\sum_{ i = 1 }^M \Tr H_i \right)^{-2} \norm{\nabla f}_2^2
\end{align}





\section{Complete Unlearning}
We assume that $f$ satisfies Assumption \ref{ass:linear_theta}.
\begin{assumption}
	\label{ass:linear_theta}
	For any data point $(\vx, \vy)$ and model with parameters $\vtheta$, 
	we consider that $f$ can be linearly approximated in $\vtheta$ for a perturbation $\vepsilon$, i.e.
	\begin{equation}
	f(\vx, \vy, \vtheta + \epsilon) 
	= f(\vx, \vy, \vtheta) + \mJ_{\vtheta}(\vx, \vy, \vtheta) \vepsilon
	,
	\end{equation}
	where $\mJ_{\vtheta}$ is the Jacobian matrix of $f$ with respect to $\vtheta$.
\end{assumption}
With Assumption \ref{ass:linear_theta} and the stochastic perturbation $\vphi$, we have
\begin{align}
	F(\vtheta + \vphi) 
	= F(\vtheta)
	+ \frac{1}{N}\sum_{ i = 1 }^{N}  \mJ_\vtheta(\vx_i, \vy_i, \vtheta) \vphi
	= F(\vtheta)
	+ \mJ_\vtheta ( \Dcal, \vtheta) \vphi
	,
\end{align}
where we define $J_\vtheta ( \Dcal, \vtheta) = \frac{1}{N}\sum_{ i = 1 }^{N}  \mJ_\vtheta(\vx_i, \vy_i, \vtheta)$ 
with a similar derivation for $F_{-\Scal}$. We remind that $\vphi \sim \mathcal{N}(\vmu, \mSigma = \mS^T \mS)$. Hence, we have
\begin{equation}
F(\vtheta + \vphi )
%\sim \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \nabla_\vtheta \Lcal( \vtheta)^T\mSigma \nabla_\vtheta \Lcal( \vtheta))
\sim \mathcal{N}( F(\vtheta) + \mJ_\vtheta (\Dcal, \vtheta)\vmu, \mJ_\vtheta ( \Dcal, \vtheta)^T\mSigma \mJ_\vtheta(\Dcal, \vtheta))
,
\end{equation}
with a similar derivation for $F_{-\Scal}$. With a non zero expected perturbation $\vmu$, a perfect unlearning can be obtained with $F(\vtheta + \vphi) = F_{-\Scal}(\vtheta + \vphi)$ by choosing $\vmu$ and $\mSigma$ such that the probability density functions of these two queries are identical. Considering the dimensions of the Jacobian, numerous $\vmu$ can satisfy this condition, we are thus interested in the ones with the smallest norm where Assumption \ref{ass:linear_theta} is the most valid. 
Hence, we have
\begin{alignat}{2}
&\min_{\vmu}        &\qquad& \norm{\vmu}^2
\\
&\text{subject to} &      & \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right]\vmu = F_{-\Scal}(\vtheta) - F(\vtheta),
\nonumber\\
&                  &      & \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right]^T\mSigma \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right] = 0 \label{eq:constraint_sigma}.
\nonumber
\end{alignat}
We define $\mJ_\vtheta(\Dcal, \Dcal_{-\Scal}) = \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right]$.
When this optimization problem is feasible, then its optimum $\vmu^*$ satisfies
\begin{equation}
	\vmu^* = \mJ_\vtheta(\Dcal, \Dcal_{-\Scal}) \left[ \mJ_\vtheta(\Dcal, \Dcal_{-\Scal})^T \mJ_\vtheta(\Dcal, \Dcal_{-\Scal})\right]^{-1} \left[F_{-\Scal}(\vtheta) - F(\vtheta)\right].
\end{equation}
Any $\Sigma$ such that equation(\ref{eq:constraint_sigma}) is satisfied works including $\mSigma =0$. Yet, considering a positive $\mSigma$ to mitigate the linear approximation would be helpful. We note that when $K=1$, we have $\mJ_\vtheta (\Dcal, \vtheta) = \nabla_\vtheta F(\vtheta)$ and can simplify the close form of $\vmu^*$ with 
\begin{equation}
\vmu^* = \frac{\nabla_\vtheta F(\vtheta) - \nabla_\vtheta F_{-\Scal}(\vtheta)}{\norm{\nabla_\vtheta F(\vtheta) - \nabla_\vtheta F_{-\Scal}(\vtheta)}^2} \left[F_{-\Scal}(\vtheta) - F(\vtheta)\right].
\end{equation}

\subsubsection{Interpretability using Local Perturbation}

Perturbating the model $\vtheta$ with $\vphi$ impacts the performance of all the data samples. As such, even with Definition \ref{def:DP_forget} only based on the data points to forget, all the samples are impacted. For interpretability concerns, we consider a local perturbation $\vpsi$ to the parameters to forget and look at the resulting pdf. 

\begin{assumption}
	For any data point $(\vx, \vy)$ and model parameters $\vtheta$, 
	we consider that $f$ can be linearly approximated in $\vx$ such that for a feature perturbation $\epsilon$ we have
	\begin{equation}
	f(\vx+ \vepsilon, \vy, \vtheta ) 
	= f(\vx, \vy, \vtheta) 
	+ J_\vx (\vx, \vy, \vtheta) \vepsilon
	,
	\end{equation}
	where $\mJ_{\vx}$ is the Jacobian matrix of $f$ with respect to $\vx$.
\end{assumption}

We consider clients are given the same Gaussian Noise $\vpsi \sim N(\vnu, \mPhi)$ which gives the following optimization problem and results $\vnu^*$. 
\begin{equation}
F(\Dcal, \vtheta)
= F(\vtheta) + \frac{1}{|\Dcal|}\sum_{ i \in S} \mJ_{\vx} (\vx_i, \vy_i, \vtheta)\vpsi
= F(\vtheta) + \frac{|\Scal|}{|\Dcal|}\mJ_{\vx} (\Dcal_\Scal, \vtheta) \vpsi 
\end{equation}
and
\begin{alignat}{2}
&\min_{\vnu}        &\qquad& \norm{\vnu}^2
\\
&\text{subject to} &      & \mJ_\vx (\Dcal_\Scal, \vtheta)\vnu  = F_{-\Scal}(\vtheta) - F(\vtheta) + \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\vmu^*,
\nonumber%\nonumber\\
%&                  &      & \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right]^T\mSigma \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right] = 0 \label{eq:constraint_sigma}.
%\nonumber
\end{alignat}


\begin{equation}
\vnu^* 
= \frac{|\Dcal|}{|\Scal|}\mJ_\vx(\Dcal_\Scal, \vtheta)
\left[ \mJ_\vx(\Dcal_\Scal, \vtheta)^T \mJ_\vx(\Dcal_\Scal, \vtheta)\right]^{-1} \left[F_{-\Scal}(\vtheta) - F(\vtheta) - \mJ_\vtheta(\Dcal_{-\Scal}, \vtheta)\vmu^* \right].
\end{equation}



We can also give every client their own perturbation $\vpsi_i \sim N(\vnu_i, \mPhi_i)$ which gives the following optimization problem and results $\vnu_i^*$.
\begin{equation}
F(\Dcal, \vtheta)
= F(\vtheta) + \frac{1}{|\Dcal|}\sum_{ i \in S} \mJ_{\vx} (\vx_i, \vy_i, \vtheta)\vpsi_i
\end{equation}
which gives the following optimization problem
\begin{alignat}{2}
&\min_{\vnu_i}        &\qquad& \frac{1}{|\Scal|}\sum_{ i \in S}\norm{\vnu_i}^2
\\
&\text{subject to} &      & \frac{1}{|\Dcal|}\sum_{ i \in \Scal} \mJ_\vx (\vx_i, \vy_i, \vtheta) \vnu_i  = F_{-\Scal}(\vtheta) - F(\vtheta) + \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\vmu^*,
\nonumber%\nonumber\\
%&                  &      & \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right]^T\mSigma \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right] = 0 \label{eq:constraint_sigma}.
%\nonumber
\end{alignat}


\begin{equation}
\vnu_i^* 
= |\Dcal| \mJ_\vx(\vx_i, \vy_i, \vtheta)
\left[ \sum_{ i \in S} \mJ_\vx(\vx_i, \vy_i, \vtheta)^T \mJ_\vx(\vx_i, \vy_i, \vtheta)\right]^{-1} \left[F_{-\Scal}(\vtheta) - F(\vtheta) - \mJ_\vtheta(\Dcal_{-\Scal}, \vtheta)\vmu^* \right].
\end{equation}




\section{Differential Privacy}

Let us consider 


\begin{equation}
\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} 
\sim \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \nabla_\vtheta \Lcal( \vtheta)^T\mSigma \nabla_\vtheta \Lcal( \vtheta))
= \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \norm{S \nabla_\vtheta \Lcal( \vtheta)}^2)
.
\end{equation}

We provide sufficient conditions for $\vmu$ and $\mS$ such that $\vtheta + \vphi$ satisfies Definition \ref{def:DP_forget}.  
$\vphi$ is a multinomial Gaussian distribution $\vphi \sim \mathcal{N}(\vmu, \mS^T \mS)$. Therefore,
\begin{equation}
\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} 
\sim \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \nabla_\vtheta \Lcal( \vtheta)^T\mSigma \nabla_\vtheta \Lcal( \vtheta))
= \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \norm{S \nabla_\vtheta \Lcal( \vtheta)}^2)
.
\end{equation}

We are investigating the probability, given that the database is $\mathcal{D}$, of observing an output that occurs with a very different probability under $\mathcal{D}$ than under and adjacent database $\Dcal_{-\Scal}$, where the probability space is $\mathbb{R}^d$. 
We define $\Delta \Lcal (\vtheta) = \Lcal(\vtheta) - \Lcal_{-\Scal}(\vtheta)$ and the privacy loss $R$ as 
\begin{equation}
R(\xi)
%\coloneqq \ln \left[ \frac{\mathbb{P}\left(\Lcal(\vtheta + \vphi) = \Lcal(\vtheta) + \xi \right)}{\mathbb{P}\left(\Lcal_{-N}(\vtheta + \vphi) = \Lcal(\vtheta) + \xi \right)} \right] 
%= \ln \left[ \frac{ \mathbb{P} \left(\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} = \xi \right)}
%{\mathbb{P} \left(\inner{\nabla_\vtheta \Lcal_{-N}( \vtheta) }{\vphi} = \Delta \Lcal (\vtheta) + \xi \right)} \right] 
\coloneqq \ln \left[ \frac{\mathbb{P}\left(\Lcal(\vtheta + \vphi) = \xi \right)}{\mathbb{P}\left(\Lcal_{-N}(\vtheta + \vphi) = \xi \right)} \right] 
= \ln \left[ \frac{ \mathbb{P} \left(\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} = \xi - \Lcal(\vtheta) \right)}
{\mathbb{P} \left(\inner{\nabla_\vtheta \Lcal_{-N}( \vtheta) }{\vphi} = \xi - \Lcal_{-N}(\vtheta)\right)} \right] 
.
\end{equation}
The numerator in the ratio describes the probability of seeing $\Lcal(\vtheta) + \xi$ when the database is $\mathcal{D}$, the denominator corresponds to the probability of seeing this same value when the database is $\Dcal_{-\Scal}$. 

$\vphi$ is a multinomial Gaussian distribution $\vphi \sim \mathcal{N}(\vmu, \mS^T \mS)$. Therefore,
\begin{equation}
	\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} 
	\sim \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \nabla_\vtheta \Lcal( \vtheta)^T\mSigma \nabla_\vtheta \Lcal( \vtheta))
	= \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \norm{S \nabla_\vtheta \Lcal( \vtheta)}^2)
	.
\end{equation}
Therefore, we have
\begin{equation}
\mathbb{P}\left(\Lcal(\vtheta + \vphi) = \xi \right)
=
\left[2 \pi \norm{ \mS \nabla_\vtheta \Lcal( \vtheta)}^2 \right]^{-1/2} e^{ - \frac{1}{2} \left(\xi - \nabla_\vtheta \Lcal(\vtheta)^T \vmu \right)^2 \norm{ \mS \nabla_\vtheta \Lcal( \vtheta)}^{-2}}
.
\end{equation}
With similar results for $\Lcal_{-\Scal}$. We can thus rewrite the privacy loss $R$ as 
\begin{align}
R 
& = \ln \left[ \frac{ \norm{ \mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}}
{\norm{\mS \nabla_\vtheta \Lcal( \vtheta)}} \right] 
+ \frac{1}{2} \left[ \left(\frac{\xi - \Lcal_{-N}(\vtheta) - \nabla_\vtheta \Lcal_{-N}(\vtheta)^T \vmu}{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}}\right)^2 
- \left(\frac{\xi - \Lcal(\vtheta) - \nabla_\vtheta \Lcal(\vtheta)^T \vmu}{\norm{\mS \nabla_\vtheta \Lcal( \vtheta)}}\right)^2  \right]
\end{align}


We define $Q \coloneqq \frac{ \norm{ \mS \nabla_\vtheta \Lcal( \vtheta)}}
{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}} $. 

\subsubsection*{$Q = 1 $}


We define $\alpha(\Lcal, \vtheta) \coloneqq \frac{\Lcal(\vtheta) - \nabla_\vtheta \Lcal(\vtheta)^T \vmu}{\norm{\mS \nabla_\vtheta \Lcal( \vtheta)}}$.
Therefore, we can simplify $R(\xi)$ as
\begin{align}
R (\xi)
& = 
\left[\alpha(\Lcal, \vtheta) - \alpha(\Lcal_{-\Scal}, \vtheta)\right]\xi 
+ 
\frac{1}{2} \left[\alpha^2(\Lcal_{-\Scal}, \vtheta) 
- \alpha^2(\Lcal, \vtheta) \right]
\end{align}

Therefore, we have $R(\xi) \le \epsilon$ when 
\begin{equation}
	R(\xi) \le \epsilon 
	\Leftrightarrow
	\xi \le \frac{\epsilon - \frac{1}{2} \left[\alpha^2(\Lcal_{-\Scal}, \vtheta) 
		- \alpha^2(\Lcal, \vtheta) \right]}
	{\alpha(\Lcal, \vtheta) - \alpha(\Lcal_{-\Scal}, \vtheta)}
	\eqqcolon \xi_1
\end{equation}


Let us assume that $\xi_1 > 0$.
To satisfy DP privacy, it suffices
\begin{equation}
	\mathbb{P}(\Lcal(\vtheta + \vphi) > \xi_1)
	\le \mathbb{P}(\inner{\nabla_\vtheta \Lcal(\vtheta)}{\vphi} > \xi_1 - \Lcal(\vtheta))
\end{equation}




We define $Q \coloneqq \frac{ \norm{ \mS \nabla_\vtheta \Lcal( \vtheta)}}
{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}} $, $U \coloneqq \Delta \Lcal (\vtheta) 
+ \left[ \nabla_\vtheta \Lcal(\vtheta)  - \nabla_\vtheta \Lcal_{-N}(\vtheta) \right]^T \vmu $,
$
S_1 = 
\{
\xi \ | \ R(\xi) \le \epsilon
\}$
, and 
$
S_2 = 
\{
\xi \ | \ R(\xi) \ge - \epsilon
\}$
.

\subsubsection*{1st case}



We change variable for ease of writing. We set $y = (\xi - \Lcal(\vtheta) - \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}) / \norm{\mS \nabla \Lcal (\vtheta)}$ which gives $\xi = \norm{\mS \nabla_\vtheta \Lcal (\vtheta)} y + \Lcal(\vtheta) + \nabla_\vtheta \Lcal( \vtheta)^T \vmu $. We also consider $U_{-N} = \frac{1}{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)} } U$. 
\begin{align}
R 
& = - \ln Q 
+ \frac{1}{2} \left[ \left(Q y +  U_{-N} \right)^2 
- y^2  \right]
\end{align}
which can be developed as 
\begin{align}
R 
& = \frac{1}{2}\left[Q^2 - 1\right] y^2
+ U_{-N} Q y
+ \frac{1}{2}U_{-N}^2
- \ln Q 
\end{align}
To find $S_1$, we consider $R_\epsilon$ defined as
\begin{align}
R_{\epsilon}
& = \frac{1}{2}\left[Q^2 - 1\right] y^2
+ \Delta(\vtheta) Q y
+ \frac{1}{2}\Delta^2(\vtheta)
- \ln Q 
-  \epsilon
.
\end{align}
We define $\Delta_{\epsilon}$ the associated characteristic polynomial of $R_\epsilon$, i.e.
\begin{equation}
\Delta_{ \epsilon}
= U_{-N}^2 Q^2 - 4 \frac{1}{2}\left[Q^2 - 1\right]\left[\frac{1}{2}U_{-N}^2 - \ln Q - \epsilon\right]
= U_{-N}^2 + 2\left[Q^2 - 1\right]\left[\ln Q + \epsilon\right]
\end{equation}
Let us call $y_1$ and $y_2$ the two roots of $\Delta_{\epsilon}$ such that $y_{1} < y_{2}$. 
Therefore, we have
\begin{equation}
y_{1}
= \frac{- \Delta(\vtheta) Q - \sqrt{\Delta_{\epsilon}}}{Q^2 - 1}
\text{ and }
y_{2}
= \frac{- \Delta(\vtheta) Q + \sqrt{\Delta_{\epsilon}}}{Q^2 - 1}
.
\end{equation}
Therefore, we have
\begin{equation}
	S_1 
	= \left[
	\xi_1 \coloneqq \norm{\mS \nabla_\vtheta \Lcal (\vtheta)} y_1 + \nabla_\vtheta \Lcal( \vtheta)^T \vmu, 
	\xi_2 
	\coloneqq \norm{\mS \nabla_\vtheta \Lcal (\vtheta)} y_2 + \nabla_\vtheta \Lcal( \vtheta)^T \vmu
	\right]
\end{equation}

We consider that $\Delta$ is such that $y_1 < 0$ and $y_2>0$. 
For DP to be satisfied,we want 
\begin{equation}
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \notin S_1
\right)
\le \delta
\Leftrightarrow
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \le \xi_1
\right)
+
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \ge \xi_2
\right)
\le \delta
\end{equation}

Let us consider $X \sim N(\mu, \sigma)$, then we have 
\begin{equation}
	p(X < x ) \le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )} \text{for} x <0
\end{equation}
\begin{equation}
p(X > x ) \le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )} \text{for} x >0
\end{equation}

We can bound the cumulative distribution function of a normal distribution using the complementary error function which gives
\begin{equation}
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \le \xi_1
\right)
+
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \ge \xi_2
\right)
\le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )}
+ \sqrt{2}\sigma\frac{e^{-(x_2 - \mu)^2/2 \sigma^2}}{2 (x_2 - \mu_1 )}
\end{equation}


Finally, for DP to be satisfied,we want 
\begin{equation}
	\mathbb{P}
	\left( 
	\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)\in S_1
	\right)
	\ge 1- \delta
\end{equation}




\subsubsection*{2nd case}



We change variable for ease of writing. We set 
$z = (\xi - \Lcal_{-N}(\vtheta) - \inner{\nabla_\vtheta \Lcal_{-N}( \vtheta)}{\vmu}) / \norm{\mS \nabla \Lcal_{-N} (\vtheta)}$ 
which gives 
$\xi = \norm{\mS \nabla_\vtheta \Lcal_{-N} (\vtheta)} z + \Lcal_{-N}(\vtheta) + \inner{\nabla_\vtheta \Lcal_{-N}( \vtheta)} {\vmu} $. 
We also consider $\frac{1}{\norm{\mS \nabla_\vtheta \Lcal( \vtheta)} } U 
= \frac{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}}{\norm{\mS \nabla_\vtheta \Lcal( \vtheta)} } \frac{1}{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}}U
= \frac{1}{Q}U_{-N}$. 

\begin{align}
R 
& = - \ln Q
+ \frac{1}{2} \left[ z^2 
- \left( \frac{1}{Q} z - \frac{1}{Q} U_{-N} \right)^2 \right]
\end{align}
which we can develop as 
\begin{align}
R 
& = \frac{1}{2}\left[1 - \frac{1}{Q^2}\right] z^2 
+ \frac{1}{Q^2} U_{-N} z
- \ln Q
- \frac{1}{2}  \frac{1}{Q^2}U_{-N}^2
\end{align}

We define $\Delta_{\epsilon}$ the associated characteristic polynomial of $R_\epsilon$, i.e.
\begin{equation}
\Delta_{ \epsilon}
= \frac{1}{Q^4} U_{-N}^2  
- 4 \frac{1}{2}\left[ 1 - \frac{1}{Q^2}\right]\left[- \frac{1}{2}\frac{1}{Q^2}U_{-N}^2 - \ln Q + \epsilon\right]
= \frac{1}{Q^2} U_{-N}^2 + 2\left[1 - \frac{1}{Q^2}\right]\left[\ln Q - \epsilon\right]
\end{equation}
Let us call $y_1$ and $y_2$ the two roots of $\Delta_{\epsilon}$ such that $y_{1} < y_{2}$. 
Therefore, we have
\begin{equation}
y_{1}
= \frac{- \Delta(\vtheta) Q - \sqrt{\Delta_{\epsilon}}}{Q^2 - 1}
\text{ and }
y_{2}
= \frac{- \Delta(\vtheta) Q + \sqrt{\Delta_{\epsilon}}}{Q^2 - 1}
.
\end{equation}
Therefore, we have
\begin{equation}
S_1 
= \left[
\xi_1 \coloneqq \norm{\mS \nabla_\vtheta \Lcal (\vtheta)} y_1 + \nabla_\vtheta \Lcal( \vtheta)^T \vmu, 
\xi_2 
\coloneqq \norm{\mS \nabla_\vtheta \Lcal (\vtheta)} y_2 + \nabla_\vtheta \Lcal( \vtheta)^T \vmu
\right]
\end{equation}

We consider that $\Delta$ is such that $y_1 < 0$ and $y_2>0$. 
For DP to be satisfied,we want 
\begin{equation}
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \notin S_1
\right)
\le \delta
\Leftrightarrow
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \le \xi_1
\right)
+
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \ge \xi_2
\right)
\le \delta
\end{equation}

Let us consider $X \sim N(\mu, \sigma)$, then we have 
\begin{equation}
p(X < x ) \le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )} \text{for} x <0
\end{equation}
\begin{equation}
p(X > x ) \le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )} \text{for} x >0
\end{equation}

We cn bound the cumulative distribution function of a normal distribution using the complementary error function which gives
\begin{equation}
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \le \xi_1
\right)
+
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \ge \xi_2
\right)
\le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )}
+ \sqrt{2}\sigma\frac{e^{-(x_2 - \mu)^2/2 \sigma^2}}{2 (x_2 - \mu_1 )}
\end{equation}


Finally, for DP to be satisfied,we want 
\begin{equation}
\mathbb{P}
\left( 
\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)\in S_1
\right)
\ge 1- \delta
\end{equation}


%
%
%
%
%Noting that we can retrieve $\xi$ with $\xi = \norm{\mS \nabla_\vtheta \Lcal(\vtheta)} y + \nabla_\vtheta \Lcal(\vtheta)^T \vmu$.
%
%Let us define 
%\begin{equation}
%S_1 
%= \{ \Lcal(\vtheta + \xi) \text{ s.t. } \xi \in \left[ \xi_1, \xi_2 \right] \},
%S_2 
%= \{ \Lcal(\vtheta + \xi) \text{ s.t. } \xi \in \mathbb{R}\backslash \left[ \xi_1, \xi_2 \right] \},
%\text{ and } S = S_1 \cup S_2
%\end{equation}
%
%
%\begin{align}
%\mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S \right]
%&= \mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_1 \right]
%+ \mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_2 \right]
%\\
%& \le e^\epsilon \mathbb{P}\left[ \Lcal_{-N}(\vtheta + \xi) \in S_1 \right]
%+ \delta
%\\
%& \le e^\epsilon \mathbb{P}\left[ \Lcal_{-N}(\vtheta + \xi) \in S \right]
%+ \delta
%\end{align}
%
%\begin{equation}
%\mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_2 \right]
%\end{equation}
%
%
%Let us consider $X\sim N (\nu, \sigma^2)$. Using the tail bound, we get
%\begin{equation}
%\mathbb{P}(X - \nu > x) 
%\le  \frac{\sigma}{\sqrt{2 \pi}}\frac{1}{x} e^{- x^2 /2 \sigma^2}
%\end{equation}
%
%
%
%\begin{align}
%\mathbb{P}(\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} \le \xi_1)
%&\le \frac{\norm{S \nabla_\vtheta \Lcal(\vtheta)}}{\sqrt{2\pi}}\frac{1}{\xi_1 - \nabla_\vtheta \Lcal(\vtheta)^T \vmu}
%e^{-(\xi_1 - \nabla_\vtheta \Lcal(\vtheta)^T \vmu)/ 2 \norm{\mS \nabla_\vtheta \Lcal(\vtheta)}^2}
%\\
%&= \frac{1}{\sqrt{2\pi}}\frac{1}{y_1}
%e^{- 1 / 2 y_1^2 }
%\end{align}
%
%\begin{align}
%\mathbb{P}(\inner{\nabla_\vtheta \Lcal_{-N}( \vtheta) }{\vphi} \le \xi_1)
%&\le \frac{\norm{S \nabla_\vtheta \Lcal_{-N}(\vtheta)}}{\sqrt{2\pi}}\frac{1}{\xi_1 - \nabla_\vtheta \Lcal_{-N}(\vtheta)^T \vmu}
%e^{-(\xi_1 - \nabla_\vtheta \Lcal_{-N}(\vtheta)^T \vmu)/ 2 \norm{\mS \nabla_\vtheta \Lcal_{-N}(\vtheta)}^2}
%\end{align}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%We want to find 
%\begin{equation}
%	S_1 = 
%	\{
%	\xi \ | \ |R(\xi)| \le \epsilon
%	\}
%	,
%\end{equation}
%the set of $\xi$ such that we have $|R| \le \epsilon$. Therefore, we consider two functions $R_{+ \epsilon}$ and $R_{-\epsilon}$ such that
%\begin{align}
%R_{\pm \epsilon}
%& = \frac{1}{2}\left[Q^2 - 1\right] y^2
%+ \Delta(\vtheta) Q y
%+ \frac{1}{2}\Delta^2(\vtheta)
%- \ln Q 
%\pm  \epsilon
%.
%\end{align}
%We calculate there associated characteristic polynomial $\Delta_{-\epsilon}$ and $\Delta_{+\epsilon}$
%\begin{equation}
%\Delta_{\pm \epsilon}
%= \Delta(\vtheta)^2 Q^2 - 4 \frac{1}{2}\left[Q^2 - 1\right]\left[\frac{1}{2}\Delta^2(\vtheta) - \ln Q \pm \epsilon\right]
%= \Delta^2(\vtheta) + 2\left[Q^2 - 1\right]\left[\ln Q \mp \epsilon\right]
%\end{equation}
%Let us call $y_{1, +\epsilon}$ and $y_{2, +\epsilon}$ the two roots of $\Delta_{+\epsilon}$ such that $y_{1, +\epsilon} < y_{2, +\epsilon}$. Similarly, we define $y_{1, -\epsilon}$ and $y_{2, -\epsilon}$.
%Therefore, we have
%\begin{equation}
%	y_{1, \pm\epsilon}
%	= \frac{- \Delta(\vtheta) Q - \sqrt{\Delta_{\pm\epsilon}}}{Q^2 - 1}
%	\text{ and }
%	y_{2, \pm\epsilon}
%	= \frac{- \Delta(\vtheta) Q + \sqrt{\Delta_{\pm \epsilon}}}{Q^2 - 1}
%	.
%\end{equation}
%
%We note that $\Delta$ is proportional to $(Q^2 -1)\epsilon$.
%If $Q^2 - 1>0$, then we have $\Delta_{+\epsilon} \le \Delta_{-\epsilon}$ which gives $y_{1, - \epsilon} \le y_{1, + \epsilon} \le y_{2, + \epsilon} \le y_{2, - \epsilon}$.
%Lastly, $R_{\pm \epsilon}$ is negative in $[y_{1, \pm \epsilon}, y_{2, \pm \epsilon}]$ and positive otherwise. Therefore, $R + \epsilon \le 0$ on $[y_{1, + \epsilon}, y_{2, + \epsilon}]$ and $R - \epsilon \le 0$ on $[y_{1, - \epsilon}, y_{2, - \epsilon}]$.
%\begin{equation}
%	Q^2 - 1 > 0
%	\Rightarrow
%	S_1 = [y_{1, - \epsilon}, y_{1, + \epsilon}] \cup [y_{2, + \epsilon}, y_{2, - \epsilon}]
%\end{equation}
%Similarly, if $Q^2 - 1 < 0$, then we have $\Delta_{+\epsilon} \ge \Delta_{-\epsilon}$ which gives $y_{1, + \epsilon} \le y_{1, - \epsilon} \le y_{2, - \epsilon} \le y_{2, + \epsilon}$.
%Lastly, $R_{\pm \epsilon}$ is positive in $[y_{1, \pm \epsilon}, y_{2, \pm \epsilon}]$ and negative otherwise. Therefore, $R + \epsilon \ge 0$ on $[y_{1, + \epsilon}, y_{2, + \epsilon}]$ and $R - \epsilon \ge 0$ on $[y_{1, - \epsilon}, y_{2, - \epsilon}]$.
%\begin{equation}
%Q^2 - 1 < 0
%\Rightarrow
%S_1 = [y_{1, + \epsilon}, y_{1, - \epsilon}] \cup [y_{2, - \epsilon}, y_{2, + \epsilon}]
%\end{equation}
%
%
%
%
%
%
%
%
%
%Let us define $\Delta \coloneqq \min (\Delta_{-\epsilon}, \Delta_{\epsilon})$. We have
%\begin{equation}
%y_{1}
%= \frac{- \Delta(\vtheta) Q - \sqrt{\Delta}}{Q^2 - 1}
%\text{ and }
%y_{2}
%= \frac{- \Delta(\vtheta) Q + \sqrt{\Delta}}{Q^2 - 1}
%\end{equation}
%Noting that we can retrieve $\xi$ with $\xi = \norm{\mS \nabla_\vtheta \Lcal(\vtheta)} y + \nabla_\vtheta \Lcal(\vtheta)^T \vmu$.
%
%Let us define 
%\begin{equation}
%	S_1 
%	= \{ \Lcal(\vtheta + \xi) \text{ s.t. } \xi \in \left[ \xi_1, \xi_2 \right] \},
%	S_2 
%	= \{ \Lcal(\vtheta + \xi) \text{ s.t. } \xi \in \mathbb{R}\backslash \left[ \xi_1, \xi_2 \right] \},
%	\text{ and } S = S_1 \cup S_2
%\end{equation}
%
%
%\begin{align}
%	\mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S \right]
%	&= \mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_1 \right]
%	+ \mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_2 \right]
%	\\
%	& \le e^\epsilon \mathbb{P}\left[ \Lcal_{-N}(\vtheta + \xi) \in S_1 \right]
%	+ \delta
%	\\
%	& \le e^\epsilon \mathbb{P}\left[ \Lcal_{-N}(\vtheta + \xi) \in S \right]
%	+ \delta
%\end{align}
%
%\begin{equation}
%	\mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_2 \right]
%\end{equation}
%
%
%Let us consider $X\sim N (\nu, \sigma^2)$. Using the tail bound, we get
%\begin{equation}
%	\mathbb{P}(X - \nu > x) 
%	\le  \frac{\sigma}{\sqrt{2 \pi}}\frac{1}{x} e^{- x^2 /2 \sigma^2}
%\end{equation}
%
%
%
%\begin{align}
%	\mathbb{P}(\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} \le \xi_1)
%	&\le \frac{\norm{S \nabla_\vtheta \Lcal(\vtheta)}}{\sqrt{2\pi}}\frac{1}{\xi_1 - \nabla_\vtheta \Lcal(\vtheta)^T \vmu}
%	e^{-(\xi_1 - \nabla_\vtheta \Lcal(\vtheta)^T \vmu)/ 2 \norm{\mS \nabla_\vtheta \Lcal(\vtheta)}^2}
%	\\
%	&= \frac{1}{\sqrt{2\pi}}\frac{1}{y_1}
%	e^{- 1 / 2 y_1^2 }
%\end{align}
%
%\begin{align}
%\mathbb{P}(\inner{\nabla_\vtheta \Lcal_{-N}( \vtheta) }{\vphi} \le \xi_1)
%&\le \frac{\norm{S \nabla_\vtheta \Lcal_{-N}(\vtheta)}}{\sqrt{2\pi}}\frac{1}{\xi_1 - \nabla_\vtheta \Lcal_{-N}(\vtheta)^T \vmu}
%e^{-(\xi_1 - \nabla_\vtheta \Lcal_{-N}(\vtheta)^T \vmu)/ 2 \norm{\mS \nabla_\vtheta \Lcal_{-N}(\vtheta)}^2}
%\end{align}













\subsubsection{Interpretability with local perturbation}

Perturbating the model $\vtheta$ with $\vphi$ impacts the performance of all the data samples. As such, even with Definition \ref{def:DP_forget} only based on the data points to forget, all the samples are impacted. For interpretability concerns, we consider a local perturbation $\vpsi$ to the parameters to forget and look at the resulting pdf. 

We also consider the following linear approximation

\begin{assumption}
	For any data point $(\vx, \vy)$ and model with parameters $\vtheta$, 
	we consider that $l$ can be linearly approximated in $\vx$, i.e.
	\begin{equation}
	l(\vx+ \vepsilon, \vy, \vtheta ) = l(\vx, \vy, \vtheta) + \nabla_\vx l(\vx, \vy, \vtheta) \vepsilon
	,
	\end{equation}
	with $\norm{\vepsilon} \ll \norm{\vx}$.
\end{assumption}

Therefore, we consider
\begin{equation}
	\Lcal(\Dcal, \vtheta)
	= \Lcal(\vtheta) + \frac{1}{|\Dcal|}\sum_{ i \in S} \inner{\nabla_\vx l(\vx_i, \vy_i, \vtheta)}{\vpsi_i}
\end{equation}


\subsection{Practical Implementation}











==> tex/initialization.tex <==
\subsection{Influence of the initial model on the bias}

Let us consider $X$ the feature matrix and $Y$ the ground truth with loss function 
\begin{equation}
	f(\vtheta) = \frac{1}{N} \frac{1}{2} \left[\mY - \mX \vtheta \right]^T \left[\mY - \mX \vtheta \right]
\end{equation}
We assume that there are more features than data samples. Therefore, $X^TX$ is singular and all the model $\vtheta^*$ satisfying
\begin{equation}
	\mX^T \mX \vtheta^* = \mX^T \mY
\end{equation}
are optimal model. $f$ is non convex. 

The SGD process can be rewritten such that 
\begin{equation}
	\vtheta^N 
	= \underbrace{\left[I - \eta \mX^T \mX\right]^N}_{A(\mX, N)} \vtheta^0 
	+ \underbrace{\eta \sum_{n =0}^{N-1} \left[I - \eta \mX^T \mX\right]^n \mX^T \mY}_{B(\mX, \mY, N)}
\end{equation}
We consider a learning rate small enough such that the highest eigen value of $\mX^T \mX$ is strictly inferior to 1. We also consider that its smallest eigen value is non-negative. Therefore, $I - \eta \mX^T \mX $ is positive definite. We get
\begin{equation}
\vtheta^N 
= \underbrace{\left[I - \eta \mX^T \mX\right]^N}_{A(\mX, N)} \vtheta^0 
+ \underbrace{\eta \sum_{n =0}^{N-1} \left[I - \eta \mX^T \mX\right]^n \mX^T \mY}_{B(\mX, \mY, N)}
\end{equation}

The second term is independent from the initial model and only depends of the amount of SGD $N$. When $\mX^T\mX$ i non singular, the first term converges to 0.

We differentiate now 2 flows. One with all the samples and another one with one removed sample.

\begin{equation}
\vtheta_2^N 
= A(\mX_2, N) \vtheta^0 
+ B(\mX_2,  \mY_2, N)
\end{equation}

If unlearning with $\tilde{N}$ SGD, we have
\begin{align}
\tilde{\vtheta}_2^{\tilde{N}} 
&= A(\mX_2, \tilde{N}) \vtheta_1^N 
+ B(\mX_2,  \mY_2, \tilde{N})
\\
&= A(\mX_2, \tilde{N}) \left[A(\mX_1, N) \vtheta^0 
+ B(\mX_1,  \mY_1, N)\right]
+ B(\mX_2,  \mY_2, \tilde{N})
\\
&= A(\mX_2, \tilde{N}) A(\mX_1, N) \vtheta^0 
+ A(\mX_2, \tilde{N}) B(\mX_1,  \mY_1, N)
+ B(\mX_2,  \mY_2, \tilde{N})
\end{align}

We always have 
\begin{equation}
	\lim_{\tilde{N} \to \infty} 
	B(\mX_2,  \mY_2, \tilde{N})
	=
	\lim_{N \to \infty} 
	B(\mX_2,  \mY_2, N)
\end{equation}
and if $\mX_2^T \mX_2$ is non singular, we retrieve 
\begin{equation}
	\lim_{\tilde{N} \to \infty} 
	A(\mX_2,  \tilde{N})
	=0
\end{equation}
which gives 
\begin{align}
\lim_{\tilde{N} \to \infty} 
\tilde{\vtheta}_2^{\tilde{N}}
=
\lim_{N \to \infty} 
\vtheta_2^N
\end{align}

In practice, in Machine Learning, the initial model $\vtheta_0$ is obtained with a normal distribution. Setting the initial model at $0$ enables to cancel the first step, still, the second term cannot be mitigated by setting the initial model to a certain value and depends of the optimum of the previous optimum model.



==> tex/new_initial_model.tex <==

\section{New Initial Model}

Let us consider $N_t$ the SGD budget for training and $N_m$ the SGD budget for adapting the model.

DP privacy relies on noising the last model such that for any combination of samples, a model cannot know whether a sample was used to train it or not. 

We have an history of models $N_t$ models. How to obtain a new model forgetting a given data samples?

What kind of procedure can be proposed to train the learning model such that a sample is forgotten?

The method currently used is to retrain everything. Why ? Because the initial model has no information on the sample to forget. We propose in this work instead to have a better starting point  than the initial model to obtain the new model when trying to forget some samples. 

We propose a generalization of DP-Privacy. With DP, only one training is needed and a noise is added to prevent specific information recovery from one client. What should be the noise to ensure DP? Is DP equivalent to ensuring forgetting of a data sample?

What is the impact of the amount of samples to forget? e.g. forgetting a class.

We propose  the following two scenarios which we compare theoretically and experimentally to the following two baselines
\begin{enumerate}
	\item noising the trained model before performing the budget of SGD
	
	\item noising the model obtained after $N_t - N_m$ SGD before performing the budget of SGD
	
	\item noising the trained model with no retraining
	
	\item retraining from scratch with the available SGD budget
\end{enumerate}




==> tex/noise_params.tex <==
%\section{Noise data point to forget}
%
%DP privacy ensures that any removal dataset having the same dataset with one different data sample to have the same performances. This need is stronger than ours only needed for the removal of some specific data samples and not any of them. 
%
%Let us consider a dataset with $n$ data samples with $x_i, y_i$ where $\dim(x_i) = d$. Without loss of generality, we assume we want to forget the $n$th data point. 
%%
%%Let us consider 
%%\begin{equation}
%%	\Lcal(\vx) = \frac{1}{N}\sum_{i =1}^N l_i(\vx)
%%	\text{ and }
%%	\Lcal_{-n}(\vx) = \frac{1}{N-1}\sum_{i =1}^{N-1} l_i(\vx)
%%\end{equation}
%%
%We define $r(\vx_i, \vtheta)$ the predictions of model with parameters $\vtheta$ on data point $\vx_i$. 
%We define $\vepsilon_i$ the perturbation given to client features $\vx_i$.
%We consider $\vepsilon_i$ is small enough that $r$ can be linearly approximated with respect to its input. We get
%\begin{equation}
%r(\vx_i + \vepsilon_i , \vtheta)
%= r (\vx_i, \vtheta) + \nabla_\vx r(\vx_i, \vtheta)\vepsilon_i 
%\end{equation}
%The impact on the loss function can thus be expressed as
%%For ease, of writing, we write $r(\vx + \vepsilon_i) = \sum_{i =1}^N r(\vx_i + \vepsilon_i)  $
%\begin{equation}
%\norm{r(\vx_i + \epsilon_i, \vtheta) - \vy_i}^2
%= \norm{r(\vx_i, \vtheta) - \vy_i}^2
%+ 2 \inner{r(\vx_i, \vtheta) - \vy_i}{\nabla_\vx r(\vx_i, \vtheta)\epsilon_i}
%+ \norm{\nabla_\vx r(\vx_i, \vtheta)\epsilon_i}^2
%.
%\end{equation}
%We define $f(\vx, \vy, \vtheta) \coloneqq \norm{r(\vx, \vtheta) - \vy}^2$, $F(\vtheta) \coloneqq \sum_{i =1}^N f(\vx_i, \vy_i, \vtheta)$, and $G(\vtheta) \coloneqq \sum_{i =1}^N f(\vx_i + \vepsilon_i, \vy_i, \vtheta)$ 
%
%\begin{equation}
%	G(\vtheta)
%	= F (\vtheta) + \sum_{i=1}^{N} \left[2 \inner{r(\vx_i, \vtheta) - \vy_i}{\nabla_\vx r(\vx_i, \vtheta)\epsilon_i}
%	+ \norm{\nabla_\vx r(\vx_i, \vtheta)\epsilon_i}^2\right]
%\end{equation}
%
%Let us consider a linear approximation around the perturbation of $\vtheta$ with $\vphi$. We have
%\begin{equation}
%r(\vx_i, \vtheta + \vphi)
%= r (\vx_i, \vtheta) + \nabla_\vtheta r(\vx_i, \vtheta)\vphi 
%.
%\end{equation}
%We define $H(\vtheta) \coloneqq \sum_{i =1}^N f(\vx_i, \vy_i, \vtheta + \vphi)$ which gives
%\begin{equation}
%	H(\vtheta)
%	= F (\vtheta) + \sum_{i=1}^{N} \left[2 \inner{r(\vx_i, \vtheta) - \vy_i}{\nabla_\vtheta r(\vx_i, \vtheta)\vphi}
%	+ \norm{\nabla_\vtheta r(\vx_i, \vtheta)\vphi}^2\right]
%\end{equation}
%
%$H$ is what we obtain with the traditional DP-process by adding some noise $\vphi$ to the current model. 
%$G$ is the method by obfuscating the samples to forget with noise $\epsilon_i$. What to do with $G$? 
%
%We want the kept model to know the proper noise to give to the kept model to satisfy DP privacy. 

\section{Formalizing the Unlearning problem}

\subsection{Optimization}
We consider a dataset $\Dcal$ composed of $|\Dcal| = N$ data samples $(\vx_i, \vy_i)$ where $\vx_i$ is the feature vector of a data sample and $\vy_i$ its prediction or label.
For unsupervised learning, it suffices to consider that data samples in $\Dcal$ are only made with $\vx_i$. We denote by $\Scal$ the set of $S = |\Scal|$ indices we want to forget from $\Dcal$ and $\Dcal_{-\Scal} = \Dcal\backslash\{(\vx_i, \vy_i) | i \in \Scal \}$ the dataset without the forgotten data samples.

We consider a function $f$ depending on one data sample and model parameters $\vtheta$. 
For example, $f$ can be the loss of one data sample or its activation vector. We define the associated normalized functions 
\begin{equation}
F(\vtheta) \coloneqq \frac{1}{|\Dcal|} \sum_{i \in \Dcal} f(\vx_i, \vy_i, \vtheta)
\text{ and }
F_{-\Scal}(\vtheta) \coloneqq \frac{1}{|\Dcal_{-\Scal}|} \sum_{i \in \Dcal_{-\Scal}} f(\vx_i, \vy_i, \vtheta)
.
\end{equation}
We consider $F$ is a $K$ dimensional vector where $K=1$ if $f$ is the loss function of one data samples and $K$ is the amount of classes in a classification problem. 
For ease of writing, we consider $F_{-i}$ to be the resulting function when forgetting data sample $i$. 


\subsection{$(\epsilon, \delta)$-indistinguishable}

We first define $(\epsilon, \delta)$-indistinguishable in Definition \ref{def:DP_forget}.
\begin{definition}[$(\epsilon, \delta)$-indistinguishable] Let $\epsilon$ and $\delta$ be two positive real numbers. Two distributions $X$ and $Y$ are $(\epsilon, \delta)$-indistinguishable if for all subset $A \subseteq \Acal$, we have
	\label{def:DP_forget}
	\begin{equation}
	\mathbb{P}(X \in A) 
	\le e^\epsilon \mathbb{P}(Y \in A)  + \delta
	\text{ and }
	\mathbb{P}(Y \in A) 
	\le e^\epsilon \mathbb{P}(X \in A)  + \delta
	.
	\end{equation}
\end{definition}
$\vtheta$ is the $d$ dimensional vector of the trained model parameters. We consider a stochastic perturbation $\vphi \sim N( \vmu, \mSigma)$, where $\mSigma$ is positive definite and can thus be expressed as $\mSigma = \mS^T \mS$, such that $F(\vtheta + \vphi)$ and $F_{-\Scal}(\vtheta + \vphi)$ are $(\epsilon, \delta)$-indistinguishable.

Definition \ref{def:DP_forget} is linked to differential privacy(DP). With DP, we are looking at the noise $\vphi$ such that for any sample $i$, $F(\vtheta + \vphi)$ and $F_{-i}(\vtheta + \vphi)$ 
are $(\epsilon, \delta)$-indistinguishable. In that case, no information specific to any data sample can be retrieve from $\hat{\vtheta} \coloneqq \vtheta + \vphi$. With Machine Unlearning, we are instead looking at $\vphi$ such that $\hat{\vtheta}$ does not contain specific information from any forgotten data sample. As such, DP implies Unlearning but Unlearning is weaker than DP.

\begin{definition}[$(\epsilon, \delta, \Scal)$-unlearning] 
	If $F(\vtheta + \vphi)$ and $F_{-\Scal}(\vtheta + \vphi)$ are $(\epsilon, \delta)$-indistinguishable, $\hat{\vtheta} \coloneqq \vtheta+ \vphi$ contains no information from $\Scal$.
\end{definition}









\section{Complete Unlearning}
We assume that $f$ satisfies Assumption \ref{ass:linear_theta}.
\begin{assumption}
	\label{ass:linear_theta}
	For any data point $(\vx, \vy)$ and model with parameters $\vtheta$, 
	we consider that $f$ can be linearly approximated in $\vtheta$ for a perturbation $\vepsilon$, i.e.
	\begin{equation}
	f(\vx, \vy, \vtheta + \epsilon) 
	= f(\vx, \vy, \vtheta) + \mJ_{\vtheta}(\vx, \vy, \vtheta) \vepsilon
	,
	\end{equation}
	where $\mJ_{\vtheta}$ is the Jacobian matrix of $f$ with respect to $\vtheta$.
\end{assumption}
With Assumption \ref{ass:linear_theta} and the stochastic perturbation $\vphi$, we have
\begin{align}
	F(\vtheta + \vphi) 
	= F(\vtheta)
	+ \frac{1}{N}\sum_{ i = 1 }^{N}  \mJ_\vtheta(\vx_i, \vy_i, \vtheta) \vphi
	= F(\vtheta)
	+ \mJ_\vtheta ( \Dcal, \vtheta) \vphi
	,
\end{align}
where we define $J_\vtheta ( \Dcal, \vtheta) = \frac{1}{N}\sum_{ i = 1 }^{N}  \mJ_\vtheta(\vx_i, \vy_i, \vtheta)$ 
with a similar derivation for $F_{-\Scal}$. We remind that $\vphi \sim \mathcal{N}(\vmu, \mSigma = \mS^T \mS)$. Hence, we have
\begin{equation}
F(\vtheta + \vphi )
%\sim \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \nabla_\vtheta \Lcal( \vtheta)^T\mSigma \nabla_\vtheta \Lcal( \vtheta))
\sim \mathcal{N}( F(\vtheta) + \mJ_\vtheta (\Dcal, \vtheta)\vmu, \mJ_\vtheta ( \Dcal, \vtheta)^T\mSigma \mJ_\vtheta(\Dcal, \vtheta))
,
\end{equation}
with a similar derivation for $F_{-\Scal}$. With a non zero expected perturbation $\vmu$, a perfect unlearning can be obtained with $F(\vtheta + \vphi) = F_{-\Scal}(\vtheta + \vphi)$ by choosing $\vmu$ and $\mSigma$ such that the probability density functions of these two queries are identical. Considering the dimensions of the Jacobian, numerous $\vmu$ can satisfy this condition, we are thus interested in the ones with the smallest norm where Assumption \ref{ass:linear_theta} is the most valid. 
Hence, we have
\begin{alignat}{2}
&\min_{\vmu}        &\qquad& \norm{\vmu}^2
\\
&\text{subject to} &      & \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right]\vmu = F_{-\Scal}(\vtheta) - F(\vtheta),
\nonumber\\
&                  &      & \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right]^T\mSigma \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right] = 0 \label{eq:constraint_sigma}.
\nonumber
\end{alignat}
We define $\mJ_\vtheta(\Dcal, \Dcal_{-\Scal}) = \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right]$.
When this optimization problem is feasible, then its optimum $\vmu^*$ satisfies
\begin{equation}
	\vmu^* = \mJ_\vtheta(\Dcal, \Dcal_{-\Scal}) \left[ \mJ_\vtheta(\Dcal, \Dcal_{-\Scal})^T \mJ_\vtheta(\Dcal, \Dcal_{-\Scal})\right]^{-1} \left[F_{-\Scal}(\vtheta) - F(\vtheta)\right].
\end{equation}
Any $\Sigma$ such that equation(\ref{eq:constraint_sigma}) is satisfied works including $\mSigma =0$. Yet, considering a positive $\mSigma$ to mitigate the linear approximation would be helpful. We note that when $K=1$, we have $\mJ_\vtheta (\Dcal, \vtheta) = \nabla_\vtheta F(\vtheta)$ and can simplify the close form of $\vmu^*$ with 
\begin{equation}
\vmu^* = \frac{\nabla_\vtheta F(\vtheta) - \nabla_\vtheta F_{-\Scal}(\vtheta)}{\norm{\nabla_\vtheta F(\vtheta) - \nabla_\vtheta F_{-\Scal}(\vtheta)}^2} \left[F_{-\Scal}(\vtheta) - F(\vtheta)\right].
\end{equation}

\subsubsection{Interpretability using Local Perturbation}

Perturbating the model $\vtheta$ with $\vphi$ impacts the performance of all the data samples. As such, even with Definition \ref{def:DP_forget} only based on the data points to forget, all the samples are impacted. For interpretability concerns, we consider a local perturbation $\vpsi$ to the parameters to forget and look at the resulting pdf. 

\begin{assumption}
	For any data point $(\vx, \vy)$ and model parameters $\vtheta$, 
	we consider that $f$ can be linearly approximated in $\vx$ such that for a feature perturbation $\epsilon$ we have
	\begin{equation}
	f(\vx+ \vepsilon, \vy, \vtheta ) 
	= f(\vx, \vy, \vtheta) 
	+ J_\vx (\vx, \vy, \vtheta) \vepsilon
	,
	\end{equation}
	where $\mJ_{\vx}$ is the Jacobian matrix of $f$ with respect to $\vx$.
\end{assumption}

We consider clients are given the same Gaussian Noise $\vpsi \sim N(\vnu, \mPhi)$ which gives the following optimization problem and results $\vnu^*$. 
\begin{equation}
F(\Dcal, \vtheta)
= F(\vtheta) + \frac{1}{|\Dcal|}\sum_{ i \in S} \mJ_{\vx} (\vx_i, \vy_i, \vtheta)\vpsi
= F(\vtheta) + \frac{|\Scal|}{|\Dcal|}\mJ_{\vx} (\Dcal_\Scal, \vtheta) \vpsi 
\end{equation}
and
\begin{alignat}{2}
&\min_{\vnu}        &\qquad& \norm{\vnu}^2
\\
&\text{subject to} &      & \mJ_\vx (\Dcal_\Scal, \vtheta)\vnu  = F_{-\Scal}(\vtheta) - F(\vtheta) + \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\vmu^*,
\nonumber%\nonumber\\
%&                  &      & \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right]^T\mSigma \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right] = 0 \label{eq:constraint_sigma}.
%\nonumber
\end{alignat}


\begin{equation}
\vnu^* 
= \frac{|\Dcal|}{|\Scal|}\mJ_\vx(\Dcal_\Scal, \vtheta)
\left[ \mJ_\vx(\Dcal_\Scal, \vtheta)^T \mJ_\vx(\Dcal_\Scal, \vtheta)\right]^{-1} \left[F_{-\Scal}(\vtheta) - F(\vtheta) - \mJ_\vtheta(\Dcal_{-\Scal}, \vtheta)\vmu^* \right].
\end{equation}



We can also give every client their own perturbation $\vpsi_i \sim N(\vnu_i, \mPhi_i)$ which gives the following optimization problem and results $\vnu_i^*$.
\begin{equation}
F(\Dcal, \vtheta)
= F(\vtheta) + \frac{1}{|\Dcal|}\sum_{ i \in S} \mJ_{\vx} (\vx_i, \vy_i, \vtheta)\vpsi_i
\end{equation}
which gives the following optimization problem
\begin{alignat}{2}
&\min_{\vnu_i}        &\qquad& \frac{1}{|\Scal|}\sum_{ i \in S}\norm{\vnu_i}^2
\\
&\text{subject to} &      & \frac{1}{|\Dcal|}\sum_{ i \in \Scal} \mJ_\vx (\vx_i, \vy_i, \vtheta) \vnu_i  = F_{-\Scal}(\vtheta) - F(\vtheta) + \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\vmu^*,
\nonumber%\nonumber\\
%&                  &      & \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right]^T\mSigma \left[\mJ_\vtheta (\Dcal, \vtheta) - \mJ_\vtheta (\Dcal_{-\Scal}, \vtheta)\right] = 0 \label{eq:constraint_sigma}.
%\nonumber
\end{alignat}


\begin{equation}
\vnu_i^* 
= |\Dcal| \mJ_\vx(\vx_i, \vy_i, \vtheta)
\left[ \sum_{ i \in S} \mJ_\vx(\vx_i, \vy_i, \vtheta)^T \mJ_\vx(\vx_i, \vy_i, \vtheta)\right]^{-1} \left[F_{-\Scal}(\vtheta) - F(\vtheta) - \mJ_\vtheta(\Dcal_{-\Scal}, \vtheta)\vmu^* \right].
\end{equation}




\section{Differential Privacy}

Let us consider 


\begin{equation}
\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} 
\sim \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \nabla_\vtheta \Lcal( \vtheta)^T\mSigma \nabla_\vtheta \Lcal( \vtheta))
= \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \norm{S \nabla_\vtheta \Lcal( \vtheta)}^2)
.
\end{equation}

We provide sufficient conditions for $\vmu$ and $\mS$ such that $\vtheta + \vphi$ satisfies Definition \ref{def:DP_forget}.  
$\vphi$ is a multinomial Gaussian distribution $\vphi \sim \mathcal{N}(\vmu, \mS^T \mS)$. Therefore,
\begin{equation}
\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} 
\sim \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \nabla_\vtheta \Lcal( \vtheta)^T\mSigma \nabla_\vtheta \Lcal( \vtheta))
= \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \norm{S \nabla_\vtheta \Lcal( \vtheta)}^2)
.
\end{equation}

We are investigating the probability, given that the database is $\mathcal{D}$, of observing an output that occurs with a very different probability under $\mathcal{D}$ than under and adjacent database $\Dcal_{-\Scal}$, where the probability space is $\mathbb{R}^d$. 
We define $\Delta \Lcal (\vtheta) = \Lcal(\vtheta) - \Lcal_{-\Scal}(\vtheta)$ and the privacy loss $R$ as 
\begin{equation}
R(\xi)
%\coloneqq \ln \left[ \frac{\mathbb{P}\left(\Lcal(\vtheta + \vphi) = \Lcal(\vtheta) + \xi \right)}{\mathbb{P}\left(\Lcal_{-N}(\vtheta + \vphi) = \Lcal(\vtheta) + \xi \right)} \right] 
%= \ln \left[ \frac{ \mathbb{P} \left(\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} = \xi \right)}
%{\mathbb{P} \left(\inner{\nabla_\vtheta \Lcal_{-N}( \vtheta) }{\vphi} = \Delta \Lcal (\vtheta) + \xi \right)} \right] 
\coloneqq \ln \left[ \frac{\mathbb{P}\left(\Lcal(\vtheta + \vphi) = \xi \right)}{\mathbb{P}\left(\Lcal_{-N}(\vtheta + \vphi) = \xi \right)} \right] 
= \ln \left[ \frac{ \mathbb{P} \left(\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} = \xi - \Lcal(\vtheta) \right)}
{\mathbb{P} \left(\inner{\nabla_\vtheta \Lcal_{-N}( \vtheta) }{\vphi} = \xi - \Lcal_{-N}(\vtheta)\right)} \right] 
.
\end{equation}
The numerator in the ratio describes the probability of seeing $\Lcal(\vtheta) + \xi$ when the database is $\mathcal{D}$, the denominator corresponds to the probability of seeing this same value when the database is $\Dcal_{-\Scal}$. 

$\vphi$ is a multinomial Gaussian distribution $\vphi \sim \mathcal{N}(\vmu, \mS^T \mS)$. Therefore,
\begin{equation}
	\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} 
	\sim \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \nabla_\vtheta \Lcal( \vtheta)^T\mSigma \nabla_\vtheta \Lcal( \vtheta))
	= \mathcal{N}( \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}, \norm{S \nabla_\vtheta \Lcal( \vtheta)}^2)
	.
\end{equation}
Therefore, we have
\begin{equation}
\mathbb{P}\left(\Lcal(\vtheta + \vphi) = \xi \right)
=
\left[2 \pi \norm{ \mS \nabla_\vtheta \Lcal( \vtheta)}^2 \right]^{-1/2} e^{ - \frac{1}{2} \left(\xi - \nabla_\vtheta \Lcal(\vtheta)^T \vmu \right)^2 \norm{ \mS \nabla_\vtheta \Lcal( \vtheta)}^{-2}}
.
\end{equation}
With similar results for $\Lcal_{-\Scal}$. We can thus rewrite the privacy loss $R$ as 
\begin{align}
R 
& = \ln \left[ \frac{ \norm{ \mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}}
{\norm{\mS \nabla_\vtheta \Lcal( \vtheta)}} \right] 
+ \frac{1}{2} \left[ \left(\frac{\xi - \Lcal_{-N}(\vtheta) - \nabla_\vtheta \Lcal_{-N}(\vtheta)^T \vmu}{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}}\right)^2 
- \left(\frac{\xi - \Lcal(\vtheta) - \nabla_\vtheta \Lcal(\vtheta)^T \vmu}{\norm{\mS \nabla_\vtheta \Lcal( \vtheta)}}\right)^2  \right]
\end{align}


We define $Q \coloneqq \frac{ \norm{ \mS \nabla_\vtheta \Lcal( \vtheta)}}
{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}} $. 

\subsubsection*{$Q = 1 $}


We define $\alpha(\Lcal, \vtheta) \coloneqq \frac{\Lcal(\vtheta) - \nabla_\vtheta \Lcal(\vtheta)^T \vmu}{\norm{\mS \nabla_\vtheta \Lcal( \vtheta)}}$.
Therefore, we can simplify $R(\xi)$ as
\begin{align}
R (\xi)
& = 
\left[\alpha(\Lcal, \vtheta) - \alpha(\Lcal_{-\Scal}, \vtheta)\right]\xi 
+ 
\frac{1}{2} \left[\alpha^2(\Lcal_{-\Scal}, \vtheta) 
- \alpha^2(\Lcal, \vtheta) \right]
\end{align}

Therefore, we have $R(\xi) \le \epsilon$ when 
\begin{equation}
	R(\xi) \le \epsilon 
	\Leftrightarrow
	\xi \le \frac{\epsilon - \frac{1}{2} \left[\alpha^2(\Lcal_{-\Scal}, \vtheta) 
		- \alpha^2(\Lcal, \vtheta) \right]}
	{\alpha(\Lcal, \vtheta) - \alpha(\Lcal_{-\Scal}, \vtheta)}
	\eqqcolon \xi_1
\end{equation}


Let us assume that $\xi_1 > 0$.
To satisfy DP privacy, it suffices
\begin{equation}
	\mathbb{P}(\Lcal(\vtheta + \vphi) > \xi_1)
	\le \mathbb{P}(\inner{\nabla_\vtheta \Lcal(\vtheta)}{\vphi} > \xi_1 - \Lcal(\vtheta))
\end{equation}




We define $Q \coloneqq \frac{ \norm{ \mS \nabla_\vtheta \Lcal( \vtheta)}}
{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}} $, $U \coloneqq \Delta \Lcal (\vtheta) 
+ \left[ \nabla_\vtheta \Lcal(\vtheta)  - \nabla_\vtheta \Lcal_{-N}(\vtheta) \right]^T \vmu $,
$
S_1 = 
\{
\xi \ | \ R(\xi) \le \epsilon
\}$
, and 
$
S_2 = 
\{
\xi \ | \ R(\xi) \ge - \epsilon
\}$
.

\subsubsection*{1st case}



We change variable for ease of writing. We set $y = (\xi - \Lcal(\vtheta) - \inner{\nabla_\vtheta \Lcal( \vtheta)}{\vmu}) / \norm{\mS \nabla \Lcal (\vtheta)}$ which gives $\xi = \norm{\mS \nabla_\vtheta \Lcal (\vtheta)} y + \Lcal(\vtheta) + \nabla_\vtheta \Lcal( \vtheta)^T \vmu $. We also consider $U_{-N} = \frac{1}{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)} } U$. 
\begin{align}
R 
& = - \ln Q 
+ \frac{1}{2} \left[ \left(Q y +  U_{-N} \right)^2 
- y^2  \right]
\end{align}
which can be developed as 
\begin{align}
R 
& = \frac{1}{2}\left[Q^2 - 1\right] y^2
+ U_{-N} Q y
+ \frac{1}{2}U_{-N}^2
- \ln Q 
\end{align}
To find $S_1$, we consider $R_\epsilon$ defined as
\begin{align}
R_{\epsilon}
& = \frac{1}{2}\left[Q^2 - 1\right] y^2
+ \Delta(\vtheta) Q y
+ \frac{1}{2}\Delta^2(\vtheta)
- \ln Q 
-  \epsilon
.
\end{align}
We define $\Delta_{\epsilon}$ the associated characteristic polynomial of $R_\epsilon$, i.e.
\begin{equation}
\Delta_{ \epsilon}
= U_{-N}^2 Q^2 - 4 \frac{1}{2}\left[Q^2 - 1\right]\left[\frac{1}{2}U_{-N}^2 - \ln Q - \epsilon\right]
= U_{-N}^2 + 2\left[Q^2 - 1\right]\left[\ln Q + \epsilon\right]
\end{equation}
Let us call $y_1$ and $y_2$ the two roots of $\Delta_{\epsilon}$ such that $y_{1} < y_{2}$. 
Therefore, we have
\begin{equation}
y_{1}
= \frac{- \Delta(\vtheta) Q - \sqrt{\Delta_{\epsilon}}}{Q^2 - 1}
\text{ and }
y_{2}
= \frac{- \Delta(\vtheta) Q + \sqrt{\Delta_{\epsilon}}}{Q^2 - 1}
.
\end{equation}
Therefore, we have
\begin{equation}
	S_1 
	= \left[
	\xi_1 \coloneqq \norm{\mS \nabla_\vtheta \Lcal (\vtheta)} y_1 + \nabla_\vtheta \Lcal( \vtheta)^T \vmu, 
	\xi_2 
	\coloneqq \norm{\mS \nabla_\vtheta \Lcal (\vtheta)} y_2 + \nabla_\vtheta \Lcal( \vtheta)^T \vmu
	\right]
\end{equation}

We consider that $\Delta$ is such that $y_1 < 0$ and $y_2>0$. 
For DP to be satisfied,we want 
\begin{equation}
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \notin S_1
\right)
\le \delta
\Leftrightarrow
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \le \xi_1
\right)
+
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \ge \xi_2
\right)
\le \delta
\end{equation}

Let us consider $X \sim N(\mu, \sigma)$, then we have 
\begin{equation}
	p(X < x ) \le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )} \text{for} x <0
\end{equation}
\begin{equation}
p(X > x ) \le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )} \text{for} x >0
\end{equation}

We can bound the cumulative distribution function of a normal distribution using the complementary error function which gives
\begin{equation}
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \le \xi_1
\right)
+
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \ge \xi_2
\right)
\le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )}
+ \sqrt{2}\sigma\frac{e^{-(x_2 - \mu)^2/2 \sigma^2}}{2 (x_2 - \mu_1 )}
\end{equation}


Finally, for DP to be satisfied,we want 
\begin{equation}
	\mathbb{P}
	\left( 
	\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)\in S_1
	\right)
	\ge 1- \delta
\end{equation}




\subsubsection*{2nd case}



We change variable for ease of writing. We set 
$z = (\xi - \Lcal_{-N}(\vtheta) - \inner{\nabla_\vtheta \Lcal_{-N}( \vtheta)}{\vmu}) / \norm{\mS \nabla \Lcal_{-N} (\vtheta)}$ 
which gives 
$\xi = \norm{\mS \nabla_\vtheta \Lcal_{-N} (\vtheta)} z + \Lcal_{-N}(\vtheta) + \inner{\nabla_\vtheta \Lcal_{-N}( \vtheta)} {\vmu} $. 
We also consider $\frac{1}{\norm{\mS \nabla_\vtheta \Lcal( \vtheta)} } U 
= \frac{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}}{\norm{\mS \nabla_\vtheta \Lcal( \vtheta)} } \frac{1}{\norm{\mS \nabla_\vtheta \Lcal_{-N}( \vtheta)}}U
= \frac{1}{Q}U_{-N}$. 

\begin{align}
R 
& = - \ln Q
+ \frac{1}{2} \left[ z^2 
- \left( \frac{1}{Q} z - \frac{1}{Q} U_{-N} \right)^2 \right]
\end{align}
which we can develop as 
\begin{align}
R 
& = \frac{1}{2}\left[1 - \frac{1}{Q^2}\right] z^2 
+ \frac{1}{Q^2} U_{-N} z
- \ln Q
- \frac{1}{2}  \frac{1}{Q^2}U_{-N}^2
\end{align}

We define $\Delta_{\epsilon}$ the associated characteristic polynomial of $R_\epsilon$, i.e.
\begin{equation}
\Delta_{ \epsilon}
= \frac{1}{Q^4} U_{-N}^2  
- 4 \frac{1}{2}\left[ 1 - \frac{1}{Q^2}\right]\left[- \frac{1}{2}\frac{1}{Q^2}U_{-N}^2 - \ln Q + \epsilon\right]
= \frac{1}{Q^2} U_{-N}^2 + 2\left[1 - \frac{1}{Q^2}\right]\left[\ln Q - \epsilon\right]
\end{equation}
Let us call $y_1$ and $y_2$ the two roots of $\Delta_{\epsilon}$ such that $y_{1} < y_{2}$. 
Therefore, we have
\begin{equation}
y_{1}
= \frac{- \Delta(\vtheta) Q - \sqrt{\Delta_{\epsilon}}}{Q^2 - 1}
\text{ and }
y_{2}
= \frac{- \Delta(\vtheta) Q + \sqrt{\Delta_{\epsilon}}}{Q^2 - 1}
.
\end{equation}
Therefore, we have
\begin{equation}
S_1 
= \left[
\xi_1 \coloneqq \norm{\mS \nabla_\vtheta \Lcal (\vtheta)} y_1 + \nabla_\vtheta \Lcal( \vtheta)^T \vmu, 
\xi_2 
\coloneqq \norm{\mS \nabla_\vtheta \Lcal (\vtheta)} y_2 + \nabla_\vtheta \Lcal( \vtheta)^T \vmu
\right]
\end{equation}

We consider that $\Delta$ is such that $y_1 < 0$ and $y_2>0$. 
For DP to be satisfied,we want 
\begin{equation}
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \notin S_1
\right)
\le \delta
\Leftrightarrow
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \le \xi_1
\right)
+
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \ge \xi_2
\right)
\le \delta
\end{equation}

Let us consider $X \sim N(\mu, \sigma)$, then we have 
\begin{equation}
p(X < x ) \le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )} \text{for} x <0
\end{equation}
\begin{equation}
p(X > x ) \le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )} \text{for} x >0
\end{equation}

We cn bound the cumulative distribution function of a normal distribution using the complementary error function which gives
\begin{equation}
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \le \xi_1
\right)
+
\mathbb{P}
\left( 
%\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)
\eta_1 \ge \xi_2
\right)
\le \sqrt{2}\sigma\frac{e^{-(x_1 - \mu)^2/2 \sigma^2}}{2 (\mu_1 - x_1 )}
+ \sqrt{2}\sigma\frac{e^{-(x_2 - \mu)^2/2 \sigma^2}}{2 (x_2 - \mu_1 )}
\end{equation}


Finally, for DP to be satisfied,we want 
\begin{equation}
\mathbb{P}
\left( 
\Lcal(\vtheta + \vphi ) - \Lcal(\vtheta)\in S_1
\right)
\ge 1- \delta
\end{equation}


%
%
%
%
%Noting that we can retrieve $\xi$ with $\xi = \norm{\mS \nabla_\vtheta \Lcal(\vtheta)} y + \nabla_\vtheta \Lcal(\vtheta)^T \vmu$.
%
%Let us define 
%\begin{equation}
%S_1 
%= \{ \Lcal(\vtheta + \xi) \text{ s.t. } \xi \in \left[ \xi_1, \xi_2 \right] \},
%S_2 
%= \{ \Lcal(\vtheta + \xi) \text{ s.t. } \xi \in \mathbb{R}\backslash \left[ \xi_1, \xi_2 \right] \},
%\text{ and } S = S_1 \cup S_2
%\end{equation}
%
%
%\begin{align}
%\mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S \right]
%&= \mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_1 \right]
%+ \mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_2 \right]
%\\
%& \le e^\epsilon \mathbb{P}\left[ \Lcal_{-N}(\vtheta + \xi) \in S_1 \right]
%+ \delta
%\\
%& \le e^\epsilon \mathbb{P}\left[ \Lcal_{-N}(\vtheta + \xi) \in S \right]
%+ \delta
%\end{align}
%
%\begin{equation}
%\mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_2 \right]
%\end{equation}
%
%
%Let us consider $X\sim N (\nu, \sigma^2)$. Using the tail bound, we get
%\begin{equation}
%\mathbb{P}(X - \nu > x) 
%\le  \frac{\sigma}{\sqrt{2 \pi}}\frac{1}{x} e^{- x^2 /2 \sigma^2}
%\end{equation}
%
%
%
%\begin{align}
%\mathbb{P}(\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} \le \xi_1)
%&\le \frac{\norm{S \nabla_\vtheta \Lcal(\vtheta)}}{\sqrt{2\pi}}\frac{1}{\xi_1 - \nabla_\vtheta \Lcal(\vtheta)^T \vmu}
%e^{-(\xi_1 - \nabla_\vtheta \Lcal(\vtheta)^T \vmu)/ 2 \norm{\mS \nabla_\vtheta \Lcal(\vtheta)}^2}
%\\
%&= \frac{1}{\sqrt{2\pi}}\frac{1}{y_1}
%e^{- 1 / 2 y_1^2 }
%\end{align}
%
%\begin{align}
%\mathbb{P}(\inner{\nabla_\vtheta \Lcal_{-N}( \vtheta) }{\vphi} \le \xi_1)
%&\le \frac{\norm{S \nabla_\vtheta \Lcal_{-N}(\vtheta)}}{\sqrt{2\pi}}\frac{1}{\xi_1 - \nabla_\vtheta \Lcal_{-N}(\vtheta)^T \vmu}
%e^{-(\xi_1 - \nabla_\vtheta \Lcal_{-N}(\vtheta)^T \vmu)/ 2 \norm{\mS \nabla_\vtheta \Lcal_{-N}(\vtheta)}^2}
%\end{align}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%We want to find 
%\begin{equation}
%	S_1 = 
%	\{
%	\xi \ | \ |R(\xi)| \le \epsilon
%	\}
%	,
%\end{equation}
%the set of $\xi$ such that we have $|R| \le \epsilon$. Therefore, we consider two functions $R_{+ \epsilon}$ and $R_{-\epsilon}$ such that
%\begin{align}
%R_{\pm \epsilon}
%& = \frac{1}{2}\left[Q^2 - 1\right] y^2
%+ \Delta(\vtheta) Q y
%+ \frac{1}{2}\Delta^2(\vtheta)
%- \ln Q 
%\pm  \epsilon
%.
%\end{align}
%We calculate there associated characteristic polynomial $\Delta_{-\epsilon}$ and $\Delta_{+\epsilon}$
%\begin{equation}
%\Delta_{\pm \epsilon}
%= \Delta(\vtheta)^2 Q^2 - 4 \frac{1}{2}\left[Q^2 - 1\right]\left[\frac{1}{2}\Delta^2(\vtheta) - \ln Q \pm \epsilon\right]
%= \Delta^2(\vtheta) + 2\left[Q^2 - 1\right]\left[\ln Q \mp \epsilon\right]
%\end{equation}
%Let us call $y_{1, +\epsilon}$ and $y_{2, +\epsilon}$ the two roots of $\Delta_{+\epsilon}$ such that $y_{1, +\epsilon} < y_{2, +\epsilon}$. Similarly, we define $y_{1, -\epsilon}$ and $y_{2, -\epsilon}$.
%Therefore, we have
%\begin{equation}
%	y_{1, \pm\epsilon}
%	= \frac{- \Delta(\vtheta) Q - \sqrt{\Delta_{\pm\epsilon}}}{Q^2 - 1}
%	\text{ and }
%	y_{2, \pm\epsilon}
%	= \frac{- \Delta(\vtheta) Q + \sqrt{\Delta_{\pm \epsilon}}}{Q^2 - 1}
%	.
%\end{equation}
%
%We note that $\Delta$ is proportional to $(Q^2 -1)\epsilon$.
%If $Q^2 - 1>0$, then we have $\Delta_{+\epsilon} \le \Delta_{-\epsilon}$ which gives $y_{1, - \epsilon} \le y_{1, + \epsilon} \le y_{2, + \epsilon} \le y_{2, - \epsilon}$.
%Lastly, $R_{\pm \epsilon}$ is negative in $[y_{1, \pm \epsilon}, y_{2, \pm \epsilon}]$ and positive otherwise. Therefore, $R + \epsilon \le 0$ on $[y_{1, + \epsilon}, y_{2, + \epsilon}]$ and $R - \epsilon \le 0$ on $[y_{1, - \epsilon}, y_{2, - \epsilon}]$.
%\begin{equation}
%	Q^2 - 1 > 0
%	\Rightarrow
%	S_1 = [y_{1, - \epsilon}, y_{1, + \epsilon}] \cup [y_{2, + \epsilon}, y_{2, - \epsilon}]
%\end{equation}
%Similarly, if $Q^2 - 1 < 0$, then we have $\Delta_{+\epsilon} \ge \Delta_{-\epsilon}$ which gives $y_{1, + \epsilon} \le y_{1, - \epsilon} \le y_{2, - \epsilon} \le y_{2, + \epsilon}$.
%Lastly, $R_{\pm \epsilon}$ is positive in $[y_{1, \pm \epsilon}, y_{2, \pm \epsilon}]$ and negative otherwise. Therefore, $R + \epsilon \ge 0$ on $[y_{1, + \epsilon}, y_{2, + \epsilon}]$ and $R - \epsilon \ge 0$ on $[y_{1, - \epsilon}, y_{2, - \epsilon}]$.
%\begin{equation}
%Q^2 - 1 < 0
%\Rightarrow
%S_1 = [y_{1, + \epsilon}, y_{1, - \epsilon}] \cup [y_{2, - \epsilon}, y_{2, + \epsilon}]
%\end{equation}
%
%
%
%
%
%
%
%
%
%Let us define $\Delta \coloneqq \min (\Delta_{-\epsilon}, \Delta_{\epsilon})$. We have
%\begin{equation}
%y_{1}
%= \frac{- \Delta(\vtheta) Q - \sqrt{\Delta}}{Q^2 - 1}
%\text{ and }
%y_{2}
%= \frac{- \Delta(\vtheta) Q + \sqrt{\Delta}}{Q^2 - 1}
%\end{equation}
%Noting that we can retrieve $\xi$ with $\xi = \norm{\mS \nabla_\vtheta \Lcal(\vtheta)} y + \nabla_\vtheta \Lcal(\vtheta)^T \vmu$.
%
%Let us define 
%\begin{equation}
%	S_1 
%	= \{ \Lcal(\vtheta + \xi) \text{ s.t. } \xi \in \left[ \xi_1, \xi_2 \right] \},
%	S_2 
%	= \{ \Lcal(\vtheta + \xi) \text{ s.t. } \xi \in \mathbb{R}\backslash \left[ \xi_1, \xi_2 \right] \},
%	\text{ and } S = S_1 \cup S_2
%\end{equation}
%
%
%\begin{align}
%	\mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S \right]
%	&= \mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_1 \right]
%	+ \mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_2 \right]
%	\\
%	& \le e^\epsilon \mathbb{P}\left[ \Lcal_{-N}(\vtheta + \xi) \in S_1 \right]
%	+ \delta
%	\\
%	& \le e^\epsilon \mathbb{P}\left[ \Lcal_{-N}(\vtheta + \xi) \in S \right]
%	+ \delta
%\end{align}
%
%\begin{equation}
%	\mathbb{P}\left[ \Lcal(\vtheta + \xi) \in S_2 \right]
%\end{equation}
%
%
%Let us consider $X\sim N (\nu, \sigma^2)$. Using the tail bound, we get
%\begin{equation}
%	\mathbb{P}(X - \nu > x) 
%	\le  \frac{\sigma}{\sqrt{2 \pi}}\frac{1}{x} e^{- x^2 /2 \sigma^2}
%\end{equation}
%
%
%
%\begin{align}
%	\mathbb{P}(\inner{\nabla_\vtheta \Lcal( \vtheta) }{\vphi} \le \xi_1)
%	&\le \frac{\norm{S \nabla_\vtheta \Lcal(\vtheta)}}{\sqrt{2\pi}}\frac{1}{\xi_1 - \nabla_\vtheta \Lcal(\vtheta)^T \vmu}
%	e^{-(\xi_1 - \nabla_\vtheta \Lcal(\vtheta)^T \vmu)/ 2 \norm{\mS \nabla_\vtheta \Lcal(\vtheta)}^2}
%	\\
%	&= \frac{1}{\sqrt{2\pi}}\frac{1}{y_1}
%	e^{- 1 / 2 y_1^2 }
%\end{align}
%
%\begin{align}
%\mathbb{P}(\inner{\nabla_\vtheta \Lcal_{-N}( \vtheta) }{\vphi} \le \xi_1)
%&\le \frac{\norm{S \nabla_\vtheta \Lcal_{-N}(\vtheta)}}{\sqrt{2\pi}}\frac{1}{\xi_1 - \nabla_\vtheta \Lcal_{-N}(\vtheta)^T \vmu}
%e^{-(\xi_1 - \nabla_\vtheta \Lcal_{-N}(\vtheta)^T \vmu)/ 2 \norm{\mS \nabla_\vtheta \Lcal_{-N}(\vtheta)}^2}
%\end{align}













\subsubsection{Interpretability with local perturbation}

Perturbating the model $\vtheta$ with $\vphi$ impacts the performance of all the data samples. As such, even with Definition \ref{def:DP_forget} only based on the data points to forget, all the samples are impacted. For interpretability concerns, we consider a local perturbation $\vpsi$ to the parameters to forget and look at the resulting pdf. 

We also consider the following linear approximation

\begin{assumption}
	For any data point $(\vx, \vy)$ and model with parameters $\vtheta$, 
	we consider that $l$ can be linearly approximated in $\vx$, i.e.
	\begin{equation}
	l(\vx+ \vepsilon, \vy, \vtheta ) = l(\vx, \vy, \vtheta) + \nabla_\vx l(\vx, \vy, \vtheta) \vepsilon
	,
	\end{equation}
	with $\norm{\vepsilon} \ll \norm{\vx}$.
\end{assumption}

Therefore, we consider
\begin{equation}
	\Lcal(\Dcal, \vtheta)
	= \Lcal(\vtheta) + \frac{1}{|\Dcal|}\sum_{ i \in S} \inner{\nabla_\vx l(\vx_i, \vy_i, \vtheta)}{\vpsi_i}
\end{equation}


\subsection{Practical Implementation}











==> tex/not_kept.tex <==
%\input{./tex/review_litterature}

%\input{./tex/initialization}
%\input{./tex/problem}
%\input{./tex/alternative_SGD}
%\input{./tex/convergence}
%\input{./tex/expansion}
%\input{./tex/new_initial_model}
%\input{./tex/acknowledgements}

==> tex/other.tex <==


\subsection{A more general case}

Let us consider that clients loss functions are $\mu$ strongly convex. We denote by $\vtheta^*$ and $\vtheta_{-k}^*$ respectively the optimum of the loss function with all the clients and all but client $k$. We can obtain the following convergence guarantees
\begin{equation}
	\norm{\vtheta^N - \vtheta^*}^2 
	\le ( 1 - \eta \mu)^N \norm{\vtheta^0 - \vtheta^*}^2
\end{equation}
As such, we have
\begin{equation}
	\norm{\vtheta_{-k}^N - \vtheta^N} 
	\le 
	\norm{\vtheta_{-k}^N - \vtheta_{-k}^*} 
	+ \norm{\vtheta^N - \vtheta^*} 
	+ \norm{\vtheta_{-k}^* - \vtheta^*} 
\end{equation}
which gives
\begin{align}
\norm{\vtheta_{-k}^N - \vtheta^N} 
&\le 
\sqrt{2} ( 1 - \eta \mu)^{N/2} 
\max(\norm{\vtheta^0 - \vtheta^*}^2, \norm{\vtheta^0 - \vtheta_{-k}^*}^2)
\nonumber\\
&+ \norm{\vtheta_{-k}^* - \vtheta^*} 
\end{align}
While this result holds for more functions the main issue lies in the provided bound. Indeed, it depends of the new optimum which we do not know. 
























==> tex/other_applications.tex <==
\textit{Consider the case where $T_r = N_{\zeta_r}$.}

\begin{equation}
\Psi(n, m)
= \norm{\sum_{i =1}^M \left(p_i - q_i(m)\right) \vtheta_i^n }_p
,
\end{equation} 
where $p_i = n_i / (\sum_{i =1}^M n_i)$ and $q_i(m) =  n_i / (\sum_{i =1, j \neq m}^M n_i)$ for $i \neq m$, and $q_i(m) = 0$ otherwise. As a result, we have
\begin{equation}
\Psi(p, n, m)
= [1 - \frac{\sum_{i =1}^M n_i}{\sum_{i =1, j \neq m}^M n_i}]\vtheta^{n+1}
+ \frac{n_m}{\sum_{i =1, i\neq m}^M n_i}\vtheta_m^{n+1}
,
\end{equation} 
\begin{equation}
\Psi(p, n, m)
= \frac{n_m}{\sum_{i =1, i\neq m}^M n_i}\left[\vtheta_m^{n+1} - \vtheta^{n+1}\right]
,
\end{equation} 


client sampling

unlearning in centralized with shards

In term of time complexity, if we consider that our model has $d$ parameters, at one iteration, computing the noise sensitivity of one client requires $\Ocal(d)$ time complexity. Therefore computing the time complexity of every client has a time complexity of $\Ocal(Md)$. Computing the noise sensitivity does not slow-down \textsc{FedAvg}. Indeed, it can be done in parallel while clients compute their local work.

Across the learning process, the server receives $MN$ client contributions and performs $N$ server aggregations. Keeping the $N$ global models is not needed. Indeed, if the noise variance threshold $\sigma^2$ is known in advance, saving a global model per client is sufficient, i.e. saving up to $M$ different models.

\textit{Computing the sensitivity for every client has complexity $\Ocal(K)$. INCLUDE $d$.}

\textit{Machine unlearning in the centralized setting. Shards.}

==> tex/priorities.tex <==

%Include Hessian. 

%Link with differential privacy.

%Hessian + Differential privacy

%The noise is specific to every client


%Computing the sensitivity for every client has complexity $\Ocal(K)$. INCLUDE $d$.

%When working with many clients where only some of the clients can be forgotten, a client can be split in many other clients. 

%When working with too many clients,  clusters of clients can instead be created. As such, a set of clients is forgotten instead of just one. 
%Link with the cosine similarity

%Trade-off with the amount of local work $K$.

Increase computation speed

Extension to shards

Client sampling

==> tex/problem.tex <==
Most of the current Machine Unlearning (MU) literature considers the following learning setup. 
A model is trained to minimize its loss on a dataset. 
After training, the dataset is changed to either include new data points or remove already used data points. 
How to obtain the optimum of the loss function associated to this changed dataset ?

The baseline always considered is to train a new model from scratch which requires significant computation power and time.  
Instead, the model obtained with the old dataset could be modified to account for the change in loss function. However, training this model includes information from the data samples to forget. Theoretically, with an infinite amount of SGD, the new model will converge to the new optimum. Yet, in practice retraining is often constrained by a bound on the amount of SGD updates. Guarantees regarding the forgetting of deleted data samples in the resulting suboptimum point need thus to be provided. Current work propose forgetting criteria based on differential privacy (DP) or KL divergence. 

We note that a proposed algorithm needs to be faster than the baseline and needs to be able to keep good model performance after any amount of serial edits to the dataset. In that case, we speak of a stream of updates. 


Many methods propose to include anonymisation components to the learning methods which in turn degrades the trained model. 
Keeping in mind the final model performance is important. Indeed, a random model is completely private but useless. This points is only considered in \cite{DescentToDelete}. 
Current works evaluate the correctness of their algorithm by looking at the resulting testing accuracy and training loss. 
\cite{TowardsProbabilisticVerification} propose a probabilistic approach based on an adversarial attack to verify if an algorithm has forgotten some data samples or not. 

No theoretical work has currently been proposed to extend MU to the distributed setting. Like for DP or client sampling, a first approach would be to consider that every client is a data sample. Yet, transposing research conducted on forgetting data samples to forgetting clients is not straight forward. Contrarily to FL, when data is centralized the server has access to it. 

Centralized datasets are often the aggregation of datasets owned by different source. 
MU is useful for many applications including removing data samples from a corrupted source or forgetting source that used their legal write to be forgotten, e.g. GDPR. In the first case, the only goal is obtaining the new optimum while, in the second one, giving forgetting guarantees is also needed. 

Interrogations:
\begin{itemize}	
	\item Why retrain without the sample we want to forget? Why not do descents with the kept samples and ascents with the forgotten ones ?
	
	\item DP already provides privacy and thus forgetting guarantees. How to forget a client with stronger DP after a model trained with DP?
	
\end{itemize} 





==> tex/proof_diff_bound.tex <==
In this section, we provide the proof of Theorem \ref{theo:diff_bound} when considering the following Assumption \ref{ass:taylor_approx} instead of Assumption \ref{ass:linear_approx}: 

\begin{assumption}\label{ass:taylor_approx}
    For model parameters $\vtheta$ and $\vphi$, the gradient of the loss function of a given data point $\Dcal_x$ satisfies
    \begin{equation}
	\nabla f_{\Dcal_x}(\vphi)
	= \nabla f_{\Dcal_x}(\vtheta)
	+ H_{\Dcal_x}(\vtheta)(\vphi - \vtheta)
        + \Ocal(\vphi - \vtheta)
	,
    \end{equation}
    where $H_{\Dcal_x}(\vtheta)$ is positive semi-definite.
\end{assumption}

We note that Assumption \ref{ass:linear_approx} reduces to Assumption \ref{ass:taylor_approx} when assuming the the high-order terms of the Taylor expansion are null.
We first consider the case where clients perform $K=1$ SGD in Section \ref{app:subsec:proof_DL} before considering the general case $K \ge 1$ in Section \ref{app:subsec:proof_FL}.

\subsection{Proof of Theorem \ref{theo:diff_bound} for $K=1$}\label{app:subsec:proof_DL}



\begin{proof}
    We define by $\vtheta^N = \textsc{FedAvg}(I, N)$ and $\vphi^N = \textsc{FedAvg}(I_{-c}, N)$ the models trained with $\textsc{FedAvg}$ on $\vtheta_0$ with respectively all the clients, i.e. $I$, and all the clients but client $c$, i.e. $I_{-c}$, performing $K=1$ GD step.

    When clients perform $K=1$ GD step, two consecutive global models can be related, when training with clients in $I$ as a simple GD step, i.e.
    \begin{equation}
	\vtheta^{n+1}
	= \vtheta^n
	- \eta \nabla f_I(\vtheta^n)
	.
    \end{equation}
    By considering the same process for $I_{-c}$ and with Assumption \ref{ass:taylor_approx}, we get
    \begin{align}
        \vphi^{n+1} - \vtheta^{n+1}
        & = \vphi^n - \vtheta^n 
        - \eta \left[ \nabla f_{I_{-c}}(\vphi^n) - \nabla f_I(\vtheta^n) \right]
        \\
        & = \left[I - \eta H_{I_{-c}}(\vtheta^n) \right] \left[\vphi^n - \vtheta^n \right]
        - \eta \left[ \nabla f_{I_{-c}}(\vtheta^n) - \nabla f_I(\vtheta^n) \right] 
        \nonumber\\
        &+ \Ocal(\vphi^n - \vtheta^n)
	\label{eq:diff}
	.
	\end{align}
        $H_{I_{-c}}(\vtheta^n)$ is semi-positive, Assumption \ref{ass:taylor_approx}. Let us define $\sigma_\text{max} (H_{I_{-c}}(\vtheta^n))$ the highest eigenvalue of $H_{I_{-c}}(\vtheta^n)$. When consider that $\eta \le 1/\sigma_\text{max} (H_{I_{-c}}(\vtheta^n))$, and due to the subadditivity of the norm, we get the following recurrent inequality
	\begin{align}
	\norm{\vphi^{n+1} - \vtheta^{n+1}}_2
	&\le
	\eta \norm{\nabla f_I(\vtheta^n) - \nabla f_{I_{-c}}(\vtheta^n)}_2
	+ \norm{\vphi^n - \vtheta^n}_2
 + \Ocal(\norm{\vphi^n - \vtheta^n}_2)
	,
	\end{align}
 which when developed completes the proof when clients perform $K=1$ GD.
\end{proof}


\subsection{Proof of Theorem \ref{theo:diff_bound} for $K\ge 1$}\label{app:subsec:proof_FL}

\begin{proof}
    We maintain the definitions of $\vtheta^n$ and $\vphi^n$ introduced in Section \ref{app:subsec:proof_DL}. To account for the amount of local SGDs $K$, we introduce $\vtheta_i^{n , k}$ the model of client $i$ after $k$ GD steps performed on global model $\vtheta^n$. We apply a similar reasoning for $\vphi_i^{n , k}$.

    With Assumption \ref{ass:taylor_approx}, we have
    \begin{equation}
        \nabla f_i (\vphi_i^{n, k})
        = \nabla f_i (\vtheta_i^{n, k})
        + H_i  (\vtheta_i^{n, k}) \left(\vphi_i^{n, k} - \vtheta_i^{n, k}\right)
        + \Ocal(\vphi_i^{n, k} - \vtheta_i^{n, k})
        \label{eq:rewrite_linear}
        ,
    \end{equation}
    which gives
    \begin{align}
        \vphi_i^{n, k+1} - \vtheta_i^{n, k+1}
        & = \left( \vphi_i^{n, k+1} - \vphi_i^{n, k}\right) 
	- \left( \vtheta_i^{n, k+1 } - \vtheta_i^{n, k} \right)
	+ \left(\vphi_i^{n, k} - \vtheta_i^{n, k}\right)
        \\
        & = - \eta \left[\nabla f_i \left(\vphi_i^{n, k}\right) 
	- \nabla f_i \left(\vtheta_i^{n, k} \right) \right]
	+ \left(\vphi_i^{n, k} - \vtheta_i^{n, k}\right) 
	\\
	& = \left[I - \eta H_i (\vtheta_i^{n, k}) \right]\left(\vphi_i^{n, k} - \vtheta_i^{n, k}\right)
    + \Ocal(\vphi_i^{n, k} - \vtheta_i^{n, k})
	\\
	& = \left[\prod_{r=0}^{k}\left[I - \eta H_i (\vtheta_i^{n, r}) \right]\right]\left(\vphi^n - \vtheta^n \right)    
    + \sum_{r=0}^{k}\Ocal(\vphi_i^{n, r} - \vtheta_i^{n, r})
	\label{eq:diff_two_locals}
	,      
    \end{align}
    where the third equality follows from equation (\ref{eq:rewrite_linear}), and the fourth from expanding the recurrent equation. For the rest of this work, we define $Q_i^n = \prod_{k=0}^{K-1}\left[I - \eta H_i (\vtheta_i^{n, k}) \right]$ and $R_i^n = \sum_{r=0}^{K-1}\Ocal(\vphi_i^{n, r} - \vtheta_i^{n, r})$
    
    Using equation (\ref{eq:diff_two_locals}), we relate the difference between two global models with every client in $I$ and in $I_c$. When removing client $c$ the clients' importance changes. We consider importance $p_i$ when training with $I$. Instead, when training with clients in $I_c$, we consider the regularized importance $q_i = p_i / (1 - p_c)$ for the remaining clients and $q_c = 0$. Considering \textsc{FedAvg} aggregation scheme (\ref{eq:FedAvg_server_aggregation}), we have
    \begin{align}
	\vphi^{n+1} - \vtheta^{n+1}
	& = \sum_{i=1}^M q_i \vphi_i^{n+1} 
	- \sum_{i=1}^M p_i \vtheta_i^{n+1}
        \\
        & = \sum_{i=1}^M q_i \left[ \left(\vphi_i^{n+1} - \vtheta_i^{n+1}\right) + \left(\vtheta_i^{n+1} - \vtheta^n \right) \right] 
	- \sum_{i=1}^M p_i \left(\vtheta_i^{n+1} - \vtheta^n\right)
        \label{app:eq:question}\\
	& = \left(\sum_{i=1}^M q_i Q_i^n \right) \left(\vphi^n - \vtheta^n\right) + \sum_{i=1}^M q_i R_i^n
	+ \Delta(I_{-c}, \vtheta^n)
	- \Delta(I, \vtheta^n)
	,
    \label{app:eq:diff_one}
    \end{align}
      where equation (\ref{app:eq:question}) results from the fact that $\sum_{i=1}^Mq_i \vtheta^n = \sum_{i=1}^M p_i \vtheta^n =\vtheta^n $.

    We consider a learning rate $\eta$ such that $\eta \le 1/\sigma_\text{max} (H_i(\vtheta^{n , k}))$. Hence, $\norm{Q_i^n}_2 \le 1$. With equation (\ref{app:eq:diff_one}), we get the following inequality
    \begin{align}
	\norm{\vphi^{n+1} - \vtheta^{n+1}}_2
	& \le \norm{\vphi^n - \vtheta^n}_2
	+ \norm{ \Delta(I, \vtheta^n)
	- \Delta(I_{-c}, \vtheta^n)}_2
        \nonumber\\
        &+  \sum_{i=1}^M q_i \sum_{r=0}^{K-1}\Ocal(\norm{\vphi_i^{n, r} - \vtheta_i^{n, r}}_2)
	,
	%	\label{app:eq:diff_one}
    \end{align}
    which expansion completes the proof.    
	
\end{proof}


\subsection{Local Loss Functions' Regularization and Strong Convexity, Proof of Corollary \ref{cor:tighter}}
\label{app:subsec:regularization}


\begin{proof}
   Under L2 regularization, every client's regularized loss function $F_i$ is expressed as  
    \begin{equation}
        F_i(\vtheta)
        = f_i(\vtheta)
        + \frac{\lambda}{2}\norm{\vtheta}^2
	\text{ and }
	\nabla F_i(\vtheta)
	= \nabla f_i(\vtheta)
	+ \lambda\vtheta
	.
    \end{equation}

    When clients perform $K=1$ GD step, equation (\ref{app:eq:diff_one}) reduces to
    \begin{align}
	\vphi^{n+1} - \vtheta^{n+1}
	& = \eta \left[\nabla f_I(\vtheta^n) -  \nabla f_{I_{-c}}(\vtheta^n) \right] 
	+ \left[(1 - \eta \lambda) I -\eta H_{I_{-c}}(\theta^n) \right](\vphi^n - \theta^n)
%	\label{eq:recurrent}
	,
    \end{align} 
    which, if $\eta \le 1 / (\lambda + \sigma_{\max}(H_i(\vtheta^n))$, gives
    \begin{align}
	\norm{\vphi^{n+1} - \vtheta^{n+1}}_2
	&\le
	\eta \norm{\nabla f_I(\vtheta^n) - \nabla f_{I_{-c}}(\vtheta^n)}_2
	+ (1- \eta \lambda -\eta \mu)\norm{\vphi^n - \vtheta^n}_2
 \nonumber\\
    &+ \Ocal(\norm{\vphi^n - \vtheta^n}_2)
	.
    \end{align}
	
    When clients perform $K\ge 1$ GD steps, we have $ \vphi_i^{n + 1} - \vtheta_i^{n + 1} = Q_i^n \left[\vphi^n - \vtheta^n\right]$ with	
    \begin{equation}
	Q_i^n
	= \prod_{r=0}^{K-1}\left[(1 - \eta \lambda)I - \eta H_i (\vtheta_i^{n, r}) \right]
	.
    \end{equation}
    Hence, we retrieve equation (\ref{app:eq:diff_one}). We consider the local learning rate satisfy $\eta \le 1 /( \lambda + \sigma_{\max} (H_i (\vtheta^n)))$. Hence, considering that $Q_i^n$ can be bounded with the $\mu$-strong convexity of the Hessian, we get 
    \begin{align}
	\norm{\vphi^{n+1} - \vtheta^{n+1}}_2
	&\le
	(1- \eta \lambda -\eta \mu)^K \norm{\vphi^n - \vtheta^n}_2
 + \norm{\Delta(I, \vtheta^n) - \Delta(I_{-c}, \vtheta^n)}_2
    \nonumber\\
        &+  \sum_{i=1}^M q_i \sum_{r=0}^{K-1}\Ocal(\norm{\vphi_i^{n, r} - \vtheta_i^{n, r}}_2)
	.
    \end{align}
    Developing this recurrent equation completes the proof.
	
	
	
\end{proof}


\subsection{Generalization}

The proof of Theorem \ref{theo:diff_bound} can  be also extended to account for FL regularization methods \cite{FedProx, FedDane, FedDyn}, other SGD solvers \cite{Adam, AdaGrad,pmlr-v89-li19c, OnTheLienarSpeedUp, Yu_Yang_Zhu_2019, haddapour2019trading}, client sampling \cite{FedProx, OnTheConvergence, TheoryClientSampling} and/or gradient compression/quantization \cite{FedPaq, QSparse, Atomo}.

\subsection{Calculus simplification with uniform importance}

For computation purposes, we propose the following expression to estimate a client bounded sensitivity, equation (\ref{eq:def_Psi}.
When removing client $c$, each client has new importance $q_i = p_i /(1 - p_c)$ for the remaining clients and $q_c = 0$. Hence, we have
\begin{align}
	 \norm{\Delta(I, \vtheta^n) - \Delta(\vtheta^n, \Dcal_{-c})}_2
	 & = \norm{\left[\vtheta^{n+1} - \vtheta^n\right] - \left[\sum_{i=1}^{M}q_i \vtheta_i^{n+1} - \vtheta^n\right]}_2
	 \\
	 & = \norm{\vtheta^{n+1} - \frac{1}{1 - p_c}\left[\vtheta^{n+1} - p_c \vtheta_i^{n+1}\right]}_2
	 \\
	 & = \frac{p_c}{1 - p_c} \norm{ \vtheta_i^{n+1} - \vtheta^{n+1} }_2
\end{align}

In the special case where clients have identical importance, we have $p_c/(1 - p_c) = 1/ (M -1)$.







































==> tex/review_litterature.tex <==
\section{Litterature Review}
\textbf{\cite{MUnlearningviaAlgorithmicStability}.}
This paper proposes a new MU algorithm for the centralized setting. The model is retrained on a fixed amount of SGD on the new dataset.

%The authors introduce $\rho$-TV stability defined as the 
%\begin{definition}
%	We define 
%	\begin{equation}
%		TV(P, Q) \coloneqq \sup_{\text{measurable sets R}} |P(R) - Q(R)|
%	\end{equation}
%	An algorithm $\mathcal{A}$ is said to be $\rho$-TV stable if
%	\begin{equation}
%		\sup_{S, S': \Delta ( S, S') = 1} TV(\mathcal{A}(S), \mathcal{A}(S')) \le \rho
%	\end{equation}
%\end{definition}
In more details, the authors propose a forgetting definition called $\rho$-TV-stability. This definition is very interesting and this work is built around it. However, their algorithm outperforms recomputation from scratch only if $\rho < 1$ and the authors show that their method has $\rho = \frac{mT}{n}$ where $m$ is the batch size, $n$ is the number of samples, and $T$ is the SGD budget. I find this point under discussed in this work and in my opinion voluntarily hidden by setting $m = \rho n/T$ which gives $m=0$ in most cases.


\textbf{\cite{DescentToDelete}.}
This work is theoretical and propose forgetting clients by adding a noise at the end of the retraining. This work uses a privacy criteria based on DP and interestingly provides an upper bound for the probability of the resulting model to be in the neighborhood of the new optimum.

Authors also propose to train different models on slices of the split dataset before aggregating the results. However, it requires slices to have iid data distributions to prevent convergence to a sub-optimum point \cite{FedNova}. Also this method requires a lot of computation to find the appropriate dataset split. 


\textbf{\cite{FederatedUnlearning}.}
This works considers MU for the federated setting but only provides a new MU algorithm and experimental results. 
The method is based on reusing the clients update of FedAvg. Yet, no theoretical justification nor any intuition behind why to use their method is provided. 
They verify the correctness of their method on the training loss and testing accuracy of the resulting model. However, how well a client is forgotten is not considered ? 


\textbf{\cite{MachineUnlearning}.}
This work considers splitting the dataset into subset and training a model per subset. The resulting model is the aggregation of all the trained models on each subset. This can be seen as FL where $N=1$ and $K\gg 1$. Therefore for this method to give the true optimum, we need all the shards to have the same data distribution which is not possible in practice even for the iid case. This work is only experimental and does not consider this point. The experimental setting only considers the testing accuracy of their method without considering if a client has been forgotten or not.

An interesting point is to consider that every sample has not the same probability to be forgotten. As such, putting them in the same shard could be useful. While it does not solve the problems considered before, associating a forgetting probability per sampling is interesting. 


\textbf{\cite{TowardsProbabilisticVerification}.}
Very interesting work proposing a framework to verify that the samples of a given owner were removed from a given model. The framework is based on an attack scheme. The attacker modifies part of its samples and add to it a marker. Through the predictions returned for the true et modified inputs, the server is able to infer if the samples of an owner were forgotten or not.

\textbf{\cite{MU_LinearFiltration}.}
Experimental work that introduce a linear filtration to remove a class from a predictive model. The authors consider models that can be decomposed as a logistic regression and a feature extraction function. The focus of this work is for a model to forget one of its class. 


\textbf{\cite{ApproximateDataDeletion}.}
This work investigates MU for linear regression. The method proposed is based on the introduction of synthetic points for the deleted points. The method proposed by the authors is linear with the dimension of the model contrarily to current quadratic complexity. 
Authors also verify their work on \cite{TowardsProbabilisticVerification} and not just on testing and training accuracy. 
This work is not based on SGD approaches. These methods gives directly the close form of the new model.


\textbf{\cite{VariationalBayesianUnlearning}.}
This work considers the problem of unlearning a model trained with a variational Bayesian approach. They propose a new lower bound to obtain the resulting posterior when forgetting some samples. Experiments compare the posterior distance of the new posterior and the one obtained with retraining which enables to measure the forgetting guarantees of their method.


\textbf{\cite{CertifiedDataRemoval}.}
DP is used to ensure unlearning like in \cite{DescentToDelete}. The authors theoretical work assume bounded gradients and Lipschitz second derivative for samples loss function. 
Authors assume that the gradient of the trained model contains too much information about the dataset used. They thus consider adding a linear perturbation to change the optimum and thus reduce the data information in the final model.
The authors measure the effectiveness of their method on testing accuracy and norm of the gradient.

 
\textbf{\cite{Cao2015TowardsMS}.}
This paper introduces 4 MU algorithms (See Table 1). 
However no theoretical guarantees are given for any of them. Correctness of unlearning algorithms are measures by comparison of the unlearned model true and false positive with respect to the ones when retraining from scratch. 


\textbf{\cite{Golatkar_2020_CVPR}.}
Definition of forgetting data based on KL divergence. 
This paper has similar elements to \cite{VariationalBayesianUnlearning}. 
Authors consider the problem of forgetting while keeping at heart a low training loss by proposing the forgetting Lagrangian. A loss function composed of the new loss function with the remaining samples regularized with the KL divergence between the current model posterior and the theoretical one. 
The formalization of the problem is  very interesting.


\textbf{\cite{MakingAIForgetYou}.}
This work proposed two MU algorithms for the problem of k-means. No theoretical guarantees are given for any of these algorithms. Experiments are conducted in term of standard metric and does not able to know if a client has been forgotten or not. Major speed-up has to be noticed for the proposed algorithms.

\textbf{\cite{WhenMachineUnlearning}.} This work considers the amount of information that can be recovered by an attacker by using the trained and modified models.

\cite{Golatkar_2021_CVPR}

\cite{golatkar2020forgetting}

\cite{shibata2021learning}

\cite{gong2021bayesian}

\cite{wang2021federated}

\cite{DeltaGrad}

\cite{WhenMachineUnlearning}

\cite{AdaptiveMachineUnlearning}

\cite{CertifiableMchineUnlearning}

\cite{FedEraser}

\cite{zeroshotMU}



==> tex/schematic_unlearning.tex <==



% \def\stride{1} %space between arrows
% \def\a{0.5} %space between columns
% \def\b{0.25} %space between columns
% \def\c{0.5} %space between columns
% \def\d{0.25} %space between columns

% \def\rotone{-10} %space between columns
% \def\rottwo{5} %space between columns


% \def\s{1.5} %space between columns
% \def\h{-5} %height of columns
% \def\id{0} %inner sep default
% \def\i{7} %inner sep

% \begin{figure}
% 	\begin{center}
% 	\begin{tikzpicture}[scale = 1, line cap=round, line join=round, >=triangle 45, x=1cm, y=1cm]
		
		

% 		%Beginnings/Ends
% 		\node[label=above: $\vtheta^0$, inner sep = \id] (O) at (0,0){} ;
% 		\node[coordinate] (A1) at (\stride, 0.1){} ;
% 		\node[coordinate] (A2) at (2 * \stride, 0.2){} ;
% 		\node[coordinate] (A3) at (3 * \stride, 0.4){} ;
% 		\node[coordinate] (A4) at (4 * \stride, 0.9){} ;
% 		\node[coordinate] (A5) at (5 * \stride, 1.2) {} ;
		
% 		\node[coordinate] (B1) at (\stride, -0.1){} ;
% 		\node[coordinate] (B2) at (2 * \stride, -0.2){} ;
% 		\node[coordinate] (B3) at (3 * \stride, -0.3){} ;
% 		\node[coordinate] (B4) at (4 * \stride, -0.9){} ;
% 		\node[coordinate] (B5) at (5 * \stride, -1.1){} ;
		
		
% 		%Vertical Arrows
% 		\draw [line width=0.5pt, ->] (O)-- (A1);
% 		\draw [line width=0.5pt, ->] (A1)-- (A2);
% 		\draw [line width=0.5pt, ->] (A2)-- (A3);
% 		\draw [line width=0.5pt, ->] (A3)-- (A4);
% 		\draw [line width=0.5pt, ->] (A4)-- (A5);
		
% 		\draw [line width=0.5pt, ->] (O)-- (B1);
% 		\draw [line width=0.5pt, ->] (B1)-- (B2);
% 		\draw [line width=0.5pt, ->] (B2)-- (B3);
% 		\draw [line width=0.5pt, ->] (B3)-- (B4);
% 		\draw [line width=0.5pt, ->] (B4)-- (B5);
		
% 		\draw[rotate=\rotone] (A5) ellipse (\a cm and \b cm);
% 		\draw[rotate=\rotone] (A5) ellipse (2 * \a cm and 2 * \b cm);
% 		\draw[rotate=\rotone] (A5) ellipse (3 * \a cm and 3 * \b cm);
		
% 		\draw[rotate=\rottwo] (B5) ellipse (\c cm and \d cm);
% 		\draw[rotate=\rottwo] (B5) ellipse (2 * \c cm and 2 * \d cm);
% 		\draw[rotate=\rottwo] (B5) ellipse (3 * \c cm and 3 * \d cm);
		
% 	\end{tikzpicture}

% 	\end{center}
	
% 	\caption{An example of the flow of global models for four consecutive forgetting requests. }
% 	\label{fig:schematic_sim}
% \end{figure}











==> tex/unlearning_proceduree.tex <==


\begin{algorithm}
	\caption{Unlearning process}\label{euclid}
	\begin{algorithmic}[1]
		
		\For{$n$ for 0 to $N-1$ (During Learning)}
		\State The server computes $\Xi$, equation (XX).
		\EndFor
		
		To forget Client $m$
		\State Takes the most recent global model such that $\Xi \le \epsilon$.
		\State Add noise to the model
		
	\end{algorithmic}
\end{algorithm}







